DeepSplit: Scalable Verification of Deep Neural Networks via Operator Splitting

Analyzing the worst-case performance of deep neural networks against input perturbations amounts to solving a large-scale non-convex optimization problem, for which several past works have proposed convex relaxations as a promising alternative. However, even for reasonably-sized neural networks, these relaxations are not tractable, and so must be replaced by even weaker relaxations in practice. In this work, we propose a novel operator splitting method that can directly solve a convex relaxation of the problem to high accuracy, by splitting it into smaller sub-problems that often have analytical solutions. The method is modular, scales to very large problem instances, and compromises operations that are amenable to fast parallelization with GPU acceleration. We demonstrate our method in bounding the worst-case performance of large convolutional networks in image classification and reinforcement learning settings, and in reachability analysis of neural network dynamical systems.

==> OJCSYS arxiv 0708 submission/abstract.tex <==
Analyzing the worst-case performance of deep neural networks against input perturbations amounts to solving a large-scale non-convex optimization problem, for which several past works have proposed convex relaxations as a promising alternative. However, even for reasonably-sized neural networks, these relaxations are not tractable, and so must be replaced by even weaker relaxations in practice. In this work, we propose a novel operator splitting method that can directly solve a convex relaxation of the problem to high accuracy, by splitting it into smaller sub-problems that often have analytical solutions. The method is modular, scales to very large problem instances, and compromises of operations that are amenable to fast parallelization with GPU acceleration. {We demonstrate our method in bounding the worst-case performance of large convolutional networks in image classification and reinforcement learning settings, and in reachability analysis of neural network dynamical systems.
}

==> OJCSYS arxiv 0708 submission/admm.tex <==
\section{Neural network verification via operator splitting} \label{sec::Scalable Neural Network Verification via Operator Splitting}
We consider an $\ell$-layer feed-forward neural network $f(x) \colon \mathbb{R}^{n_0} \to \mathbb{R}^{n_\ell}$ described by the following recursive equations,
%
\begin{align}  \label{eq: DNN model}
    \begin{aligned}
    x_0 &= x,\\  x_{k+1} &= \phi_k(x_k), \quad  k=0,\cdots,\ell-1,\\
    f(x) &= x_{\ell}
    \end{aligned}
\end{align}
%
where $x_0 \in \mathbb{R}^{n_0}$  is the input to the neural network, $x_{k} \in \mathbb{R}^{n_k}$ is the input to the $k$-th layer, and $\phi_k \colon \mathbb{R}^{n_k} \to \mathbb{R}^{n_{k+1}}$ is the operator of the $k$-th layer, which can represent any commonly-used operator in deep networks, such as linear (convolutional) layers~\footnote{Convolution is a linear operator and conceptually it can be analyzed in the same way as for linear layers.}, MaxPooling units, and activation functions.
%This formulation can easily generalize to arbitrary computational graphs as well (i.e. residual blocks). 
%We describe this generalization in Appendix \ref{app:skip} but keep the main discussion to feed-forward networks for simplicity of presentation. 
%

Given the neural network $f$, a specification function $J \colon \mathbb{R}^{n_\ell} \mapsto \mathbb{R}$, and an input set $\mathcal{X} \subset \mathbb{R}^{n_0}$, we say that $f$ satisfies the specification $J$ if $J(f(x)) \geq 0$ for all $x \in \mathcal{X}$. This is equivalent to verifying that the optimal value of \eqref{eq: maximization problem} is non-negative. We assume $\mathcal{X} \subset \mathbb{R}^{n_0}$ is a closed convex set and $J \colon \mathbb{R}^{n_{\ell}} \to \mathbb{R} \cup \{+\infty\}$ is a convex function.
%

%As an example, consider a classification problem with $n_\ell$ classes in which $f$ is the classifier network and $C(x) = \argmax_{1 \leq i \leq n_\ell} f_i(x)$ is the classification rule for a data point $x$. Given a correctly classified $x^\star \in \mathcal{X} \subset \mathbb{R}^{n_0}$, we say that $f$ is locally robust at $x^\star$ with respect to the perturbation set $\mathcal{X}$ if $C(x)=C(x^\star)$ for all $x \in \mathcal{X}$. Verifying the local robustness at $x^\star$ then amounts to verifying that the optimal values of the following $n_\ell-1$ optimization problems
% %
% \begin{align} \label{eq:class_verify}
%     \operatorname{minimize}_{x \in \mathcal{X}} \quad f_{i^\star}(x) - f_i(x) \quad i \neq i^\star,
% \end{align}
%are non-negative, where $i^\star=C(x^\star)$ is the class index of $x^\star$. 
%
%\shaoru{Note that our formulation can be generalized to residual blocks~\cite{he2016deep} by treating the summation operation $x_{k+1} = x_k^{id} + x_k^{res}$ as a separate layer}.

%Note that this formulation easily generalizes to more general objective functions (see Appendix \ref{app:skip}). %such as $J(x,f(x))$ or $\sum_{k} J_k(x_k)$. 

% \shaoru{Note that our formulation generalizes to arbitrary computational graphs (e.g. residual blocks) and general objective functions} (\shaoru{add more explanations}).

Using the sequential representation of the neural network in \eqref{eq: DNN model}, we may rewrite the optimization problem in \eqref{eq: maximization problem} as the following constrained optimization problem,
%
\begin{equation}\label{eq: nn verification problem constrained}
\begin{aligned} 
J^\star \leftarrow \text{minimize} &\quad J(x_{\ell}) \\ 
\text{subject to } &\quad x_{k+1}=\phi_k(x_{k}), \  k=0,\cdots,\ell-1, \\ 
&\quad x_0 \in \mathcal{X},
\end{aligned}
\end{equation}
%
%To obtain a convex relaxation and compute a lower bound on $J^\star$, 
with $n:=\sum_{k=0}^{\ell} n_k$ decision variables $x_0,\cdots,x_{\ell}$.
%
We can rewrite \eqref{eq: nn verification problem constrained} equivalently as
% %
\begin{equation}\label{eq: nn verification problem constrained graph form}
\begin{aligned} 
J^\star \leftarrow \text{minimize}& \quad J(x_{\ell})  \\ \text{subject to} &\quad (x_{k},x_{k+1})\in \mathcal{G}_{\phi_k}, \ k=0,\cdots,\ell-1,  \\
& \quad x_0 \in \mathcal{X},
\end{aligned}
\end{equation}
% %
where 
$$\mathcal{G}_{\phi_k} = \{(x_k,x_{k+1}) \mid x_{k+1} = \phi_k(x_k), \ \underline{x}_k \leq x_k \leq \bar{x}_k\},$$ is the graph of $\phi_k$. Here $\underline{x}_k$ and $\bar{x}_k$ are \emph{a priori} known bounds on $x_k$ when $x_0 \in \mathcal{X}$~\footnote{See Section~\ref{sec:activation_layers} for comments on finding the bounds $\underline{x}_k$ and $\bar{x}_k$.}. 
%This problem is non-convex due to presence of nonlinear operators in the network, such as activation layers, which render the set $\mathcal{G}_{\phi_k}$ nonconvex. By over-approximating $\mathcal{G}_{\phi_k}$ by a convex set (or ideally by its convex hull), we arrive at a direct layer-wise convex relaxation of the problem. However, this relaxation cannot scale to even medium-sized neural networks. In this section, by exploiting the sequential structure of the constraints, we propose a reformulation of \eqref{eq: nn verification problem constrained} whose convex relaxation can be solved efficiently and in a scalable manner. 

The problem in \eqref{eq: nn verification problem constrained graph form} is non-convex due to presence of nonlinear operators in the network, such as activation layers, which render the set $\mathcal{G}_{\phi_k}$ nonconvex. By over-approximating $\mathcal{G}_{\phi_k}$ by a convex set (or ideally by its convex hull), we arrive at a direct layer-wise convex relaxation of the problem, {in which each two consecutive variables $(x_k,x_{k+1})$ are sequentially coupled together. Solving this relaxation directly cannot exploit this structure and is hence unable to scale to even medium-sized neural networks \cite{salman2019convex}. In this section, by exploiting the sequential structure of the constraints, and introducing auxiliary decision variables (variable splitting), we propose a reformulation of \eqref{eq: nn verification problem constrained} whose convex relaxation can be decomposed into smaller sub-problems that can be solved efficiently and in a scalable manner.} 


\subsection{Variable splitting}
%
By introducing the intermediate variables $y_k$ and $z_k$, we can rewrite \eqref{eq: nn verification problem constrained} as
% % original equations
% \begin{alignat}{3} \label{eq: verification problem split}
% J^\star \leftarrow &\text{minimize} \quad && J(x_\ell)  \\ \notag
% &\text{subject to } \quad && y_{k} = x_{k}  \quad && k=0,\cdots,\ell-1 \\ \notag
% & \quad && z_{k}=\phi_k(y_k)  \quad &&k=0,\cdots,\ell-1 \\ \notag
% & \quad && x_{k+1} = z_{k}  \quad &&k=0,\cdots,\ell-1 \\ \notag
% & \quad && x_0 \in \mathcal{X}
% \end{alignat}
%
% % compressed equations
% \begin{alignat}{3} \label{eq: verification problem split}
% J^\star \leftarrow &\text{minimize} \quad && J(x_\ell)  \\ \notag
% &\text{subject to } \quad && y_{k} = x_{k}, \  & \quad && z_{k}=\phi_k(y_k) \\ 
% & \quad && x_{k+1} = z_{k}  \quad && \\ \notag
% %& \quad &&k=0,\cdots,\ell-1, \\ \notag
% %& \quad && x_0 \in \mathcal{X}
% \end{alignat}
\begin{alignat}{3} \label{eq: verification problem split}
J^\star \leftarrow &\text{minimize} \quad && J(x_\ell)  \\ \notag
&\text{subject to } \quad && y_{k} = x_{k},  \quad && k=0,\cdots,\ell-1 \\ \notag
& \quad && z_k=\phi_k(y_k),  \quad &&k=0,\cdots,\ell-1 \\ \notag
& \quad && x_{k+1} = z_{k},  \quad &&k=0,\cdots,\ell-1 \\ \notag
& \quad && x_0 \in \mathcal{X},
\end{alignat}
%
which has now $3n-n_0-n_{\ell}$ decision variables. Intuitively, we have introduced additional ``identity layers'' between consecutive layers (see Figure \ref{fig:admm_module}). By overapproximating $\mathcal{G}_{\phi_k}$ by a convex set $\mathcal{S}_{\phi_k}$, we obtain the convex relaxation
% % original equations
\begin{alignat}{3} \label{eq: verification problem split convexified}
J_{\mathrm{relaxed}}^\star \leftarrow &\text{minimize} \quad && J(x_\ell)  \\ \notag
&\text{subject to } \quad && y_{k} = x_{k},  \quad && k=0,\cdots,\ell-1 \\ \notag
& \quad && (y_k,z_k) \in \mathcal{S}_{\phi_k},  \quad &&k=0,\cdots,\ell-1 \\ \notag
& \quad && x_{k+1} = z_{k},  \quad &&k=0,\cdots,\ell-1 \\ \notag
& \quad && x_0 \in \mathcal{X},
\end{alignat}
%
%% compressed equations
% \begin{alignat}{3} \label{eq: verification problem split convexified}
% J_{\mathrm{relaxed}}^\star \leftarrow &\text{minimize} \quad && J(x_\ell)  \\ \notag
% &\text{subject to } \quad && y_{k} = x_{k}, \ (y_k,z_k) \in \mathcal{S}_{\phi_k}, \ x_{k+1} = z_{k}, \\ \notag  
% &\quad && k=0,\cdots,\ell-1, \\ \notag
% & \quad && x_0 \in \mathcal{X},
% \end{alignat}
% \begin{alignat}{3} \label{eq: verification problem split convexified}
% J_{\mathrm{relaxed}}^\star \leftarrow &\text{minimize} \quad && J(x_\ell)  \\ \notag
% &\text{subject to } \quad && y_{k} = x_{k}, (y_k,z_k) \in \mathcal{S}_{\phi_k} , x_{k+1} = z_{k}    \quad && k=0,\cdots,\ell-1 \\ \notag
% & \quad && x_0 \in \mathcal{X},
% \end{alignat}
for which $J_{\mathrm{relaxed}}^\star \leq J^\star$. This form is known as consensus as $y_k$ and $z_{k-1}$ are just copies of the variable $x_k$. As shown below, this ``overparameterization'' allows us to split the optimization problem into smaller sub-problems that can be solved in parallel and often in closed form.  


\ifdefined\arxiv
  \def\figwidth{0.5\linewidth}
\else
  \def\figwidth{1.0\linewidth}
\fi
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{admm_module.png}
    \caption{Illustration of the network structure (top) and DeepSplit computation module for a generic layer (bottom). Adding identity layers in between the neural network layers decouples the variables $x_k$ and allows processing them independently.}
    \label{fig:admm_module}
\end{figure}


\begin{figure}
	\begin{subfigure}{0.45 \columnwidth}
		\includegraphics[width = \linewidth]{conv_relu.png}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.45 \columnwidth}
		\includegraphics[width = \linewidth]{relu_linear.png}
	\end{subfigure}
	\caption{Over-approximation of the graph of ReLU function by convex hull (left) and linear bounds (right). }
	\label{fig:conv_over_approx}
\end{figure}



% \subsection{Convex Relaxation}
% %
% The problem in \eqref{eq: verification problem split} is non-convex, typically due to non-affine equality constraints $z_{k} = \phi_k(y_k)$ imposed by the activation layers. To obtain a convex relaxation, we overapproximate the graph of each function $\phi_k$ over its operating region by a convex set $\mathcal{S}_{\phi_k}$ such that $\mathcal{G}_{\phi_k} \subseteq \mathcal{S}_{\phi_k}$. In particular, the smallest $\mathcal{S}_{\phi_k}$ is the convex hull of $\mathcal{G}_{\phi_k}$. By using this relaxation in \eqref{eq: verification problem split}, we arrive at the following convex relaxation of \eqref{eq: verification problem split}:
%
%
%In the next section, we solve \eqref{eq: verification problem split convexified} using operator splitting to derive our method, DeepSplit. 
%In the next section, we develop our method, DeepSplit, which solves \eqref{eq: verification problem split convexified} using operator splitting, specifically ADMM.
%
%
\subsection{Lagrangian relaxation and operator splitting}
%
We use $\bx=(x_0,\cdots,x_{\ell})$, $\by=(y_0,\cdots,y_{\ell-1})$ and $\bz=(z_0,\cdots,z_{\ell-1})$ to denote  the concatenated variables. By relaxing the equality constraints with Lagrangian multipliers, we define the augmented Lagrangian for \eqref{eq: verification problem split convexified} as follows,
%
\begin{equation} \label{eq: augmented lagrangian}
\begin{aligned}
\mathcal{L}(\bx,\by,\bz,\blambda,\bmu) &= J(x_{\ell}) \!+\! \sum_{k=0}^{\ell-1} \mathbb{I}_{\mathcal{S}_{\phi_k}}(y_{k}, z_{k})\!+\!\mathbb{I}_{\mathcal{X}}(x_0) \\ 
&\quad + (\rho/2)\sum_{k=0}^{\ell-1} \left( \|x_k-y_k+\lambda_k\|_2^2-\|\lambda_k\|_2^2\right) + (\rho/2)\sum_{k=0}^{\ell-1} \left( \|x_{k+1}-z_k+\mu_k\|_2^2-\|\mu_k\|_2^2\right). \end{aligned}
\end{equation}
%
where $\blambda =(\lambda_0,\cdots,\lambda_{\ell-1})$ and $\bmu = (\mu_0,\cdots,\mu_{\ell-1})$ are the scaled dual variables (by $1/\rho$) and $\rho>0$ is the augmentation constant.
%
Note that we have only relaxed the equality constraints in~\eqref{eq: verification problem split convexified}, and the constraints describing the sets $\mathcal{S}_{\phi_k}$ as well as the input set $\mathcal{X}$ are kept intact. Furthermore, the inclusion of augmentation will render the dual function differentiable, and hence, easier to optimize.
%
%Minimizing the augmented Lagrangian over the primal variables $(\bx,\by,\bz)$ will yield the dual function $d(\blambda,\bmu)$, which by weak duality, is a guaranteed lower bound on $J_{\mathrm{relaxed}}^\star$,

For the Lagrangian in \eqref{eq: augmented lagrangian}, the dual function, which provides a lower bound to $J^\star_{\relaxed}$, is given by $ g(\blambda,\bmu) = \inf_{(\bx,\by,\bz)} \ \mathcal{L}(\bx,\by,\bz,\blambda,\bmu)$. The best lower bound can then be found by maximizing the dual function. \footnote{If strong duality holds, then this best lower bound would match $J^\star_{\relaxed}$. As shown in \cite{salman2019convex}, strong duality holds under mild conditions.}
%
%
%
%
However, solving the inner problem jointly over $(\bx,\by,\bz)$ to find the dual function is as difficult as solving a direct convex relaxation of \eqref{eq: nn verification problem constrained}. Instead, we split the primal variables $(\bx,\by,\bz)$ into $\bx$ and $(\by,\bz)$ and apply the classical ADMM algorithm to obtain the following iterations (shown in Figure~\ref{fig:admm_module}) for updating the primal and dual variables,
%
\begin{subequations} \label{eq: ADMM}
	\begin{align}
	\bx^{+} &\in  \mathrm{argmin}_{\bx}\  \mathcal{L}(\bx,\by,\bz,\blambda,\bmu) \label{eq: ADMM1} \\ 
	(\by^{+},\bz^{+}) &\in  \mathrm{argmin}_{(\by,\bz)} \ \mathcal{L}(\bx^{+},\by,\bz,\blambda,\bmu) \label{eq: ADMM2} \\ 
	(\blambda^{+},\bmu^{+})&\!=\! (\blambda,\bmu) \!+\! \nabla_{(\blambda,\bmu)} \ \mathcal{L}(\bx^{+},\by^{+},\bz^{+},\blambda,\bmu). \label{eq: ADMM3}
	%\bmu^{+} &= \bmu+ \nabla_{\bmu} \ \mathcal{L}(\bx^{+},\by^{+},\bz^{+},\blambda,\bmu)
	\end{align}
\end{subequations}
%
As we show below, the Lagrangian has a separable structure by construction that can be exploited in order to efficiently implement each step of \eqref{eq: ADMM}.

\subsection{The $\bx$-update}
%
%
The Lagrangian in \eqref{eq: augmented lagrangian} is separable across the $x_k$ variables; hence, the minimization in \eqref{eq: ADMM1} can be done independently for each $x_k$. Specifically, for $k=0$, we obtain the following update rule for $x_0$,
%
\begin{subequations} \label{eq: ADMM x update breakdown}
\begin{align} \label{eq: admm first update 0}
    x_0^{+} = \proj_{\mathcal{X}}(y_0-\lambda_0).
\end{align}
%
Projections onto the $\ell_\infty$ and $\ell_2$ balls can be done in closed-form. For the $\ell_1$ ball, we can use the efficient projection scheme proposed in \cite{duchi2008efficient}, which has $\mathcal{O}(n_0)$ complexity in expectation. For subsequent layers, we obtain the updates
	\begin{align} \label{eq: admm first update}
	x_k^{+} &= \frac{1}{2}(y_k - \lambda_k + z_{k-1}-\mu_{k-1}), \ k = 1, \cdots, \ell -1, \\
	%
	x_{\ell}^{+} \!&=\! \argmin_{x_{\ell}} \ J(x_{\ell}) \!+\! \frac{\rho}{2}\|x_{\ell}\!-\!z_{\ell-1}\!+\!\mu_{\ell-1}\|_2^2.
	\end{align}
\end{subequations}
%
For convex $J$ and $\rho>0$, the optimization problem for updating $x_{\ell}$ is strongly convex with a unique optimal solution. Indeed, its solution is the proximal operator of $J/\rho$ evaluated at $z_{\ell-1}-\mu_{\ell-1}$. For the special case of linear objectives, $J(x_\ell) = c^\top x_\ell$, we obtain the closed-form solution %$x_\ell^{+} = -c/\rho + (z_{\ell-1} - \mu_{\ell-1})$.
\begin{align*}
    x_\ell^{+} = -\frac{1}{\rho} c + (z_{\ell-1} - \mu_{\ell-1}).
\end{align*}
% %

\subsection{The $(\by,\bz)$-update}
\label{sec:yz_update}
Similarly, the Lagrangian is also separable across the $(y_k,z_k)$ variables. Updating these variables in \eqref{eq: ADMM2} corresponds to the following projection operations per layer,
%
\begin{align} \label{eq:yz_proj}
(y_{k}^{+}, z_{k}^{+}) &= \proj_{\mathcal{S}_{\phi_k}}(x_k^{+} + \lambda_k, x_{k+1}^{+}+\mu_k),
%(y_{k}^{+}, z_{k}^{+})= \argmin_{(y_k,z_k)} \ (\rho/2)\| (y_k,z_k)-(x_k+\lambda_k,x_{k+1}+\mu_k)\|_2^2
\end{align}
%
for $k=0,\cdots,\ell-1$. Depending on the type of the layer (linear, activation, convolution, etc.), we obtain different projections which we describe below.
% \eric{if we need space, we can move these affine/activation layers to the appendix}
\subsubsection{Affine layers}
\label{sec:affine_layers}
Suppose $\phi_k(y_k) = W_k y_k + b_k$ is an affine layer representing a fully-connected, convolutional, or an average pooling layer. Then the graph of $\phi_k$ is already a convex set given by
%
%\begin{align}
    $\mathcal{G}_{\phi_k} = \{(y_k,z_k) \mid z_k = W_k y_k + b_k\}$. 
%\end{align}
%
%	
%Denote $\tilde{y}_k = x_k^+ + \lambda_k, \tilde{z}_k = x_{k+1}^+ + \mu_k$. 
%Then the projection $(y_k^+, z_k^+) = \proj_{\mathcal{S}_{\phi_k}}(\tilde{y}_k, \tilde{z}_k)$ in \eqref{eq:yz_proj} takes the form
%
Choosing $\mathcal{S}_{\phi_k} = \mathcal{G}_{\phi_k}$, the projection in \eqref{eq:yz_proj} takes the form
\begin{equation} \label{eq:affine_proj}
\begin{aligned}
y_k^{+} &= (I_{n_{k}} \!+\! W_k^\top W_k)^{-1}(x_k^{+}+\lambda_k \!+\! W_k^\top (x_{k+1}^{+}\!+\!\mu_k\!-\!b_k)), \\
z_k^{+} &= W_k y_k^{+} + b_k.
%y_k^+ &= W_k^\top (I + W_k W_k^\top)^{-1}(\tilde{z}_k - W_k \tilde{y}_k - b_k) + \tilde{y}_k \\
%z_k^+ &= \tilde{z}_k - (I + W_k W_k^\top)(\tilde{z}_k - W_k\tilde{y}_k - b_k).
\end{aligned}
\end{equation}
%
The matrix $(I_{n_k}+W_k^\top W_k)^{-1}$ can be pre-computed and cached for subsequent iterations. We can do this efficiently for convolutional layers using the fast Fourier transform (FFT) which we discuss in Appendix~\ref{app:convolutions} and~\ref{app:FFT}.

\subsubsection{Activation layers}
\label{sec:activation_layers}
For an activation layer of the form $\phi(x) := [\varphi_1(x_1) \ \cdots \ \varphi_{n}(x_n)]^\top$, the convex relaxation of $\mathcal{G}_{\phi}$ is given by the Cartesian product of individual convex relaxations i.e.,  $\mathcal{S}_\phi = \mathcal{S}_{\varphi_1} \times \cdots \times \mathcal{S}_{\varphi_n}$.
%
For a generic activation function $\varphi \colon \mathbb{R} \to \mathbb{R}$, suppose we have a concave upper bound $\bar{\varphi}$ and a convex lower bound $\underline{\varphi}$ on $\varphi$ over an interval $I = [\underline{x},\bar{x}]$, i.e., 
$
\underline{\varphi}(x) \leq \varphi(x) \leq \bar{\varphi}(x) \ \forall \ x \in [\underline{x},\bar{x}]$. A convex overapproximation of $\mathcal{G}_{\varphi}$ is 
%is
\begin{align}
%\mathcal{S} \! = \! \{(x,y) \mid y \geq 0, \ y \geq x, \ y \leq \underline{y} + \frac{\bar{y}-\underline{y}}{\bar{x}-\underline{x}}(x-\underline{x})\},
\mathcal{S}_{\varphi} \! = \! \{(x,y) \mid \underline{\varphi}(x) \leq y \leq \bar{\varphi}(x), \ \underline{x} \leq x \leq \bar{x} \},
\end{align}
%
which turns out to be the convex hull of  $\mathcal{G}(\varphi)$ when $\bar{\varphi}$ and $\underline{\varphi}$ are concave and convex envelopes of $\varphi$, respectively. The assumed pre-activation bounds $\underline{x}$ and $\bar{x}$ used to relax the activation functions can be obtained a priori via a variety of existing techniques such as linear bounds~\cite{kolter2017provable,zhang2018efficient,zhang2020towards} which propagate linear lower and upper bounds on each activation function (see Figure~\ref{fig:conv_over_approx}) throughout the network in a fast manner. 
% {\color{blue} In this paper, we only focus on ReLU\footnote{Rectified Linear Unit} activation layers $\phi_k(x)=\max(x,0)$.}

\begin{example}[ReLU activation function.]
\label{example:relu}
\normalfont Consider the $\relu$ activation function $\varphi(x)=\max(x,0)$ over the interval $[\underline{x},\bar{x}]$. When $\underline{x}<0<\bar{x}$, the $\relu$ function admits the envelopes $\underline \varphi(x) = \max(0,x)$, $\bar \varphi(x)= \underline{y} + \frac{\bar{y}-\underline{y}}{\bar{x}-\underline{x}}(x-\underline{x})$ on $[\underline{x}, \bar{x}]$, where $\underline{y}=\max(0,\underline{x})$ and $\bar{y}=\max(0,\bar{x})$ \cite{ehlers2017formal,kolter2017provable}. In this case, the projection of a point $(x^{(0)},y^{(0)})$ onto the convex hull of $G_\varphi$, which is a triangle shown in Figure~\ref{fig:conv_over_approx}, has a closed-form solution.
%
% 1. Active neuron ($\underline{x} \geq 0$). In this case, the convex hull is given by
% \begin{align*}
% \mathcal{S}_{\varphi} = \{(x,y) \mid y = x,\ \underline{x} \leq x \leq \bar{x} \}.
% \end{align*}
% and the projection of $(x^{(0)},y^{(0)})$ onto $\mathcal{S}_{\varphi}$ is given by $x'=y'=\min(\max(\frac{x^{(0)}+y^{(0)}}{2},\underline{x}),\bar{x})$.
%
% 2. Inactive neuron ($\bar{x}\leq 0$). In this case, the convex hull is
% %
% \begin{align*}
% \mathcal{S}_{\varphi} = \{(x,y) \mid y = 0,\ \underline{x} \leq x \leq \bar{x} \}.
% \end{align*}
% %
% and the projection of $(x^{(0)},y^{(0)})$ onto $\mathcal{S}_{\varphi}$ is given by $x'=\min(\max(x^{(0)},\underline{x}),\bar{x}),\ y'=0$.
Letting $s = \frac{\bar{y}-\underline{y}}{\bar{x}-\underline{x}}$, we first project $(x^{(0)},y^{(0)})$ onto each facet of the triangle and then select the point with the minimal distance:
%
\begin{align*}
\begin{aligned}
x^{(1)} &= \min(\max(\frac{x^{(0)}+y^{(0)}}{2},0),\bar{x}), \quad y^{(1)}= x^{(1)}, \\
x^{(2)} &= \min(\max(\frac{x^{(0)}+sy^{(0)}+s(s\underline{x}-\underline{y})}{s^2+1},\underline{x}),\bar{x}), \\
y^{(2)}&= \frac{s(x^{(0)}-\underline{x})+s^2y^{(0)}+\underline{y}}{s^2+1},\\
x^{(3)} &= \min(\max(0,x^{(0)}),\underline{x}), \quad y^{(3)}=0.
\end{aligned}
\end{align*}
The projected point is $(x',y') = (x^{(i^\star)},y^{(i^\star)})$, where $i^\star = \arg\min_{1 \leq i \leq 3} \allowdisplaybreaks \sqrt{(x^{(0)}-x^{(i)})^2+(y^{(0)}-y^{(i)})^2}$. See Figure~\ref{fig:relu_proj} for illustration. 

When either $\underline{x} \geq 0$ or $\bar{x} \leq 0$, the graph $G_\varphi$ of the ReLU function becomes a line segment which allows closed-form projection of a point. 
\end{example} 
\begin{figure}[htb]
	\centering
	\includegraphics[width = 0.5\columnwidth]{unstable_relu_proj.png}
	\caption{Projection of a point $(x_0,y_0)$ onto the convex hull of the ReLU function $y=\max(0,x)$ over the interval $[\underline{x},\bar{x}]$. We first project $(x_0,y_0)$ onto all facets of the convex hull and then select the point with minimal distance to $(x_0,y_0)$.}
	\label{fig:relu_proj}
\end{figure}

\subsection{The $(\blambda,\bmu)$-update}
%
Finally, we update the scaled dual variables as follows,
%
\begin{alignat}{2}
\begin{aligned} \label{eq:dual_update}
\lambda_{k}^{+} &= \lambda_{k} + (x_k^+ - y_k^+), \ &&k=0,\cdots,\ell-1,\\
\mu_k^{+} &= \mu_k +(x_{k+1}^{+}-z_k^{+}), \ && k=0,\cdots, \ell-1.
\end{aligned}
\end{alignat}
The DeepSplit Algorithm is summarized in Algorithm~\ref{DeepSplit Algorithm}. 

\begin{algorithm}[htb]
\SetAlgoLined
\KwData{neural network $f$ (Eq. \eqref{eq: DNN model}), bounded convex input set $\mathcal{X}$, convex function $J$.}
\KwResult{lower bound $J^\star_{\mathrm{relaxed}}$ on Problem \eqref{eq: maximization problem}.}
 \textbf{Initialization:}{ $x_0 \in \mathcal{X}$, $x_{k+1}=\phi_k(x_k)$, $y_k = x_k, \ z_k=x_{k+1}$, $\lambda_k = 0, \mu_k = 0$, $k=0,\cdots,\ell-1$, augmentation constant $\rho>0$.} \\
 \Repeat{stopping criterion is met (see Section~\ref{sec:convergence})}{
{\textbf{Step 1:} $\bx$-update \eqref{eq: ADMM x update breakdown}} \\
{ \textbf{Step 2:} $(\by,\bz)$-update \eqref{eq:yz_proj} }\\
 {\textbf{Step 3:} dual update \eqref{eq:dual_update} }
 }
 \textbf{Output:} {$J(x_\ell)$}
 \caption{DeepSplit Algorithm}
 \label{DeepSplit Algorithm}
\end{algorithm}

\subsection{Convergence and stopping criterion} \label{sec:convergence}
The DeepSplit algorithm converges to the optimal solution of the convex problem \eqref{eq: verification problem split convexified} under mild conditions. Specifically, when $J$ is closed, proper and convex, and when the sets $\mathcal{S}_k$ (convex outer approximations of the graph of the layers) along with $\mathcal{X}$ are closed and convex, we can resort to the convergence results of ADMM \cite{boyd2011distributed}. Convergence of our algorithm is formally analyzed in Appendix~\ref{app:convergence}.

Following from~\cite{boyd2011distributed}, for the LP relaxation~\eqref{eq: verification problem split convexified} of a feed-forward neural network,  the primal and dual residuals are defined as
%
\begin{equation}\label{eq:primal_residual}
\begin{aligned} 
r_p &= \sum_{k=0}^{\ell-1} \ \{\|y_{k}^{+}-x_k^{+}\|_2^2 +\|x_{k+1}^{+}-z_{k}^{+}\|_2^2\}, \\
r_{d} &= \rho \sum_{k=1}^{\ell-1} \| (y_k^{+}-y_k)  + (z_{k-1}^+ - z_{k-1}) \|_2^2  + \rho \left(\|y_{0}^{+}-y_{0}\|_2^2 + \| z_{\ell-1}^+ - z_{\ell-1} \|_2^2 \right). \notag
\end{aligned}
\end{equation}
%
These are the residuals of the optimality conditions for \eqref{eq: verification problem split convexified} and converge to zero as the algorithm proceeds.
%
A reasonable termination criterion is that the primal and dual residuals must be small, i.e. $r_p \leq \epsilon_p$ and $r_d \leq \epsilon_d$, where $\epsilon_p>0$ and $\epsilon_d>0$ are tolerance levels \cite[Chapter 3]{boyd2011distributed}. These tolerances
can be chosen using an absolute and relative criterion, such as
%%
\begin{equation*}
\begin{aligned}
\epsilon_p \!&=\! \sqrt{p} \ \epsilon_{abs} \!+\! \epsilon_{rel} \max\lbrace(\|x_0\|_2^2 \!+\! 2\sum_{i=1}^{\ell-1} \|x_i\|_2^2 \!+\! \|x_\ell\|_2^2)^{\frac{1}{2}} +(\sum_{i=0}^{\ell-1}(\| y_i\|_2^2 + \|z_i\|_2^2)^{1/2} \rbrace, \notag \\
\epsilon_d \! &=\! \sqrt{n} \ \epsilon_{abs} \! + \! \epsilon_{rel} (\|\lambda_0 \|_2^2 \!+\! \sum_{i=1}^{\ell-1} \| \lambda_i \!+\! \mu_{i-1} \|_2^2 + \|\mu_{\ell-1}\|_2^2)^{\frac{1}{2}}, \notag
\end{aligned}
\end{equation*}
%%
where $p = n_0 + 2 \sum_{i=1}^{\ell-1} n_i + n_\ell$, $n = \sum_{i=0}^\ell n_i$, $\epsilon_{abs}>0$ and $\epsilon_{rel}>0$ are absolute and relative tolerances. Here $n$ is the dimension of $\bx$, the vector of primal variables that are updated in the first step of the algorithm, and $p$ is the total number of consensus constraints. 

% For neural networks with general computational graphs such as residual networks, the primal and dual residuals as well as the stopping criteria have different representations from what is shown above. But with our proposed splitting method, these representations can be derived from~\cite[Chapter 3]{boyd2011distributed}. 

\subsection{Residual balancing for convergence acceleration}
A proper selection of the augmentation constant $\rho$ has a dramatic effect on the convergence of the ADMM algorithm. Large values of  $\rho$ enforce consensus more quickly,  yielding smaller primal residuals but larger dual ones. Conversely, smaller values of $\rho$ lead to larger primal and smaller dual residuals. Since ADMM terminates when both the primal and dual residuals are small enough, in practice we prefer to choose the augmentation parameter $\rho$ not too large or too small in order to balance the reduction in the primal and dual residuals. A commonly used heuristic to make this trade-off is residual balancing~\cite{he2000alternating}, in which the penalty parameter varies adaptively based on the following rule:
%
\begin{align*}
\rho^{+} = \begin{cases} \tau \rho & \text{ if } r_p > \mu r_d \\
\rho/\tau & \text{ if } r_d > \mu r_p 
\\
\rho & \text{otherwise},
\end{cases}
\end{align*}
where $\mu,\tau>1$ are given parameters. In our experiments, we set $\tau = 2, \mu = 10$ and found this rule to be effective in speeding up the practical convergence which is demonstrated numerically in Section~\ref{sec:expr_residual_balancing}.

% {\color{blue}
% \subsection{General neural network architecture}
% In this subsection, we sketch how our method (Algorithm~\ref{DeepSplit Algorithm}) presented above can be adapted to verify neural networks of general architectures such as recurrent neural networks (RNN) and long short-term memory (LSTM) networks. 

% For a neural network with a general architecture, following the approach used in \cite{wong2018scaling}, we can represent it as a generalized $\ell$-"layer" neural network given by the equations 
% \begin{align}
% x_{k+1} = \sum_{i=1}^{k} \phi_{ik}(x_i) \equiv \Phi_k(x_{1:k}), \quad k = 0, \cdots, \ell-1 
% \end{align}
% where $x_{1:k}$ denotes the concatenated vector of variables $(x_1, \cdots, x_k)$. 
% Note that this view of a network reduces to the feedforward equations in \eqref{eq: DNN model} when $\phi_{ik}(x_i) = 0$ for all $i < k$. Furthermore, this view subsumes arbitrary skip connections, such as residual connections. Then, the graph form of the verification problem in \eqref{eq: nn verification problem constrained graph form} can be rewritten for the generalized neural network as 
% \begin{alignat}{3}
% J^\star \leftarrow &\text{minimize} \quad && J(x_{\ell})  \\ \notag
% &\text{subject to } \quad && (x_{1:k},x_{k+1})\in \mathcal{G}_{\Phi_k}, \quad &&k=0,\cdots,\ell-1 \\ \notag
% & \quad && x_0 \in \mathcal{X}.
% \end{alignat}
% Similar to before, let $S_{\Phi_k}$ be a sound convex approximation of $\mathcal{G}_{\Phi_k}$. Then, our convex relaxation introduces additional intermediate variables $y_{1:k}^k = (y_1^k, \cdots, y_k^k)$ which are copies of $x_{1:k}$ and $z_k$ for each generalized layer $\Phi_k$ to get the following convex relaxation (analogous to \eqref{eq: verification problem split convexified}): 
% %
% \begin{alignat}{3} 
% \label{eq:generalized_LP}
% p_{\mathrm{relaxed}}^\star \leftarrow &\text{minimize} \quad && J(x_\ell)  \\ \notag
% &\text{subject to } \quad && y_{1:k}^k = x_{1:k},  \quad && k=0,\cdots,\ell-1 \\ \notag
% & \quad && (y_{1:k}^k,z_k) \in \mathcal{S}_{\Phi_k},  \quad &&k=0,\cdots,\ell-1 \\ \notag
% & \quad && x_{k+1} = z_{k},  \quad &&k=0,\cdots,\ell-1 \\ \notag
% & \quad && x_0 \in \mathcal{X}.
% \end{alignat}
% Thus, applying ADMM to solve~\eqref{eq:generalized_LP} for neural networks with arbitrary skip connections reduces to deriving the corresponding projection operator onto $\mathcal{S}_{\Phi_k}$. Since most residual connections simply add an affine transformation of a previous layer, these projections are straightforward and have a closed form.

% Note that with given pre-activation bounds, an individual convex polyhedral over-approximation of the graph of the activation function $\varphi_{ik}$ (ReLU, sigmoid, tanh, etc.) can be obtained. The projection onto such polyhedron can be implemented in closed-form similar to Example~\ref{example:relu}. Therefore, verifying RNN or LSTM is equivalent to solving~\eqref{eq:generalized_LP} for the unrolled network through ADMM for which the primal and dual residuals as well as the stopping criteria can be derived from~\cite[Chapter 3]{boyd2011distributed}. 
% }


==> OJCSYS arxiv 0708 submission/comparison.tex <==
\section{Connection to Lagrangian-based methods}
\label{sec:lagrangian}
In this section, we consider verification of the feed-forward neural network~\eqref{eq: DNN model} and draw connections to two related methods relying on Lagrangian relaxation. Specifically, we relate our approach to an earlier dual method \cite{dvijotham2018dual} (Section~\ref{sec:dj}), as well as a recent Lagrangian decomposition method  \cite{bunel2020lagrangian} (Section~\ref{sec:bunel}). Overall, these approaches use a similar Lagrangian formulation, but the specific choices in splitting and augmentation of the Lagrangian result in slower theoretical convergence guarantees when solving the convex relaxation to optimality. 
%{\color{red} Eric: suggestion: relabel section 2 as a subsection of section 1 as background material, maybe? it's kind of a short section to have its own number}
%
%
%
%  We can then either directly relax the non-convex constraints, or formulate and solve the dual problem.  We discuss these two approaches next.

\subsection{Dual method via Lagrangian relaxation of the nonconvex problem}
\label{sec:dj}
%
Instead of splitting the neural network equations~\eqref{eq: nn verification problem constrained} with auxiliary variables, an alternative strategy is to directly relax~\eqref{eq: nn verification problem constrained} with Lagrangian multipliers \cite{dvijotham2018dual}: 
%
\begin{align}
 \mathcal{L}(\bx,\blambda) \!=\! J(x_{\ell}) + \sum_{k=0}^{\ell-1} \lambda_k^\top (x_{k+1}\!-\!\phi_k(x_k)) + \mathbb{I}_{\mathcal{X}}(x_0).   
\end{align}
%
where $\bx = (x_0,\cdots,x_{\ell})$ and $\blambda = (\lambda_0,\cdots,\lambda_{\ell-1})$. This results in the dual problem $g^\star \leftarrow \text{maximize} \ g(\blambda)$, 
%
%\begin{alignat}{3} \label{eq: nn verification problem constrained 1}
%d_{O}^\star \leftarrow &\text{maximize} \quad && g(\lambda).
%\end{alignat}
%
where the dual function is
\begin{align*}
    g(\blambda) &\!=\! \inf_{\underline{x}_{\ell} \leq x_{\ell} \leq \bar{x}_{\ell}} \ \{J(x_{\ell}) + \lambda_{\ell-1}^\top x_{\ell}\} \!+\! \inf_{x_0 \in \mathcal{X}_0} \{-\lambda_0^\top \phi_0(x_0)\}  +\sum_{k=1}^{\ell-1} \inf_{\underline{x}_k \leq x_k \leq \bar{x}_k} \{\lambda_{k-1}^\top x_k \!-\! \lambda_k^\top \phi_k(x_k)\}.
\end{align*}
%
By weak duality, $g^\star \leq J^\star$. %Furthermore, the dual problem in \eqref{eq: nn verification problem constrained 1} is the dual of the convex relaxation in \eqref{} when $\mathcal{S}_{\phi_k}$ is the convex hull of $\mathcal{G}_{\phi_k}$ \cite{salman2019convex}.  
%
The inner minimization problems to compute the dual function $g(\blambda)$ for a given $\blambda$ can often be solved efficiently or even in closed-form \cite{dvijotham2018dual}. The resulting dual problem is unconstrained but non-differentiable; hence it is solved using dual subgradient method \cite{dvijotham2018dual}. However, subgradient methods are known to be very slow with convergence rate $O(1/\sqrt{N})$ where $N$ is the number of updates \cite{nesterov2003introductory}, making it inefficient to find exact solutions to the convex relaxation. On the other hand, this method can be stopped at any time to obtain a valid lower bound. 

\subsection{Lagrangian method via a non-separable splitting}
\label{sec:bunel}
%
Another related approach is the Lagrangian decomposition method from \cite{bunel2020lagrangian}. 
% Instead of splitting the convex relaxation with two sets of variables as we do in \eqref{eq: verification problem split convexified}, they instead use only one set of variables 
% Specifically, to obtain a direct convex relaxation of \eqref{eq: nn verification problem constrained}, we can overapproximate the graph of $\phi_k$ by a convex set $\mathcal{S}_{\phi_k}$ such that $\mathcal{G}_{\phi_k} \subseteq \mathcal{S}_{\phi_k}$. 
%Note that for affine operators (e.g., fully-connected or convolutional layers) the graph of the operator is already convex and no approximation is incurred for those layers. 
%
% This overapproximation leads to a layer-wise convex relaxation of \eqref{eq: nn verification problem constrained},
%
% \begin{alignat}{3} \label{eq: nn verification problem constrained graph form convex relaxation}
% J_{\mathrm{relaxed}}^\star \leftarrow &\text{minimize} \quad && J(x_{\ell})  \\ \notag
% &\text{subject to } \quad && (x_{k},x_{k+1})\in \mathcal{S}_{\phi_k} \quad &&k=0,\cdots,\ell-1 \\ \notag
% & \quad && x_0 \in \mathcal{X}.
% \end{alignat}
% %
% The optimal value of \eqref{eq: nn verification problem constrained graph form convex relaxation} is  a lower bound to the optimal value of \eqref{eq: nn verification problem constrained} ($J^\star_{\relaxed} \leq J^\star$), and the quality of this bound is directly influenced by the tightness of the relaxation. In particular, when $\mathcal{S}_{\phi_k}= \mathrm{conv}(\mathcal{G}_{\phi})$, which leads to the tightest convex relaxation, the dual of \eqref{eq: nn verification problem constrained graph form convex relaxation} will coincide with the dual problem of under mild assumptions \eqref{eq: nn verification problem constrained} \cite{dvijotham2018dual,salman2019convex}.
%
To decouple the constraints for the convex relaxation of \eqref{eq: nn verification problem constrained}, this approach can be viewed as introducing \emph{one} set of intermediate variables $y_k$ as copies of $x_k$  to obtain
%
\begin{alignat}{3} \label{eq: nn verification problem split bunel}
J_{\mathrm{relaxed}}^\star \leftarrow &\text{minimize} \quad && J(y_{\ell})  \\ \notag
&\text{subject to } \quad && (y_{k},x_{k+1})\in \mathcal{S}_{\phi_k} \quad &&k=0,\cdots,\ell-1 \\ \notag
& \quad && y_k = x_k \quad && k=0,\cdots,\ell \\ \notag
& \quad && x_0 \in \mathcal{X} \notag
\end{alignat}
%
This splitting is in the spirit of the splitting introduced in \cite{bunel2020lagrangian,bunel2020branch},\footnote{If we define $\phi_k(x_k) = W_{k+1} \sigma(x_k)+b_{k+1}$, where $W_{k+1},b_{k+1}$ are the parameters of the affine layer and $\sigma$ is a layer of activation functions, this splitting coincides with the one proposed in \cite{bunel2020lagrangian,bunel2020branch}}  and differs from our splitting which uses \emph{two} sets of variables in \eqref{eq: verification problem split}.
% Note that in contrast to our splitting in \eqref{eq: nn verification problem constrained graph form}, which uses two sets of variables to fully separate layers, this formulation only introduces one set of variables. 
By relaxing the consensus constraints $y_k=x_k$, the Lagrangian is
\begin{align} \label{eq: lagrangian of convex relaxation bunel}
    \mathcal{L}(\bx,\by,\bmu) &= J(y_{\ell}) + \sum_{k=0}^{\ell} \mu_k^\top (y_k - x_k) + \sum_{k=0}^{\ell-1} \mathbb{I}_{\mathcal{S}_{\phi_k}}(y_k,x_{k+1})+\mathbb{I}_{\mathcal{X}}(x_0).
    % \\ \notag
    % & = \underbrace{J(y_{\ell})\! +\! \mu_{\ell}^\top y_{\ell}}_{\text{function of } y_{\ell}} + \sum_{k=0}^{\ell-1} \underbrace{(\mu_k^\top y_k - \mu_{k+1}^\top x_{k+1} \!+\!\mathbb{I}_{\mathcal{S}_{\phi_k}}(y_k,x_{k+1}))}_{\text{function of } (y_k,x_{k+1})}\!\! \underbrace{-\mu_0^\top x_0 + \mathbb{I}_{\mathcal{X}}(x_0)}_{\text{function of } x_0}
\end{align}
%
Again the Lagrangian is separable and its minimization results in the following dual function
%
\begin{align*} \label{eq: dual of convex relaxation bunel}
    g(\bmu) &= \inf_{\underline{x}_{\ell} \leq y_{\ell} \leq \bar{x}_{\ell}}  \{J(y_{\ell}) + \mu_{\ell}^\top y_{\ell}\} +\inf_{x_0 \in \mathcal{X}} \{-\mu_0^\top x_0\} + \sum_{k=0}^{\ell-1} \inf_{(y_k,x_{k+1})\in \mathcal{S}_{\phi_k}} \{\mu_k^\top y_k - \mu_{k+1}^\top x_{k+1}\}. 
\end{align*}
% \cite{bunel2020lagrangian} proves that for ReLU activations, maximizing the dual in \eqref{eq: dual of convex relaxation bunel} yields bounds at least as tight as the bounds obtained by maximimzing the dual in \eqref{eq: dual function nonconvex}.

%As before, the Lagrangian in \eqref{eq: lagrangian of convex relaxation bunel} is separable across the primal variables, and hence, can be minimized efficiently.
Since the dual function is not differentiable, it must be maximized by a subgradient method, which again has an $O(1/\sqrt{N})$ rate. To induce differentiability in the dual function and improve speed, \cite{bunel2020lagrangian} uses augmented Lagrangian. Since only one set of variables was introduced in \eqref{eq: nn verification problem split bunel}, the augmented Lagrangian is no longer separable across the primal variables. 
%
Therefore, for each update of the dual variable, the augmented Lagrangian must be minimized iteratively. To this end, \cite{bunel2020lagrangian} uses the Frank-Wolfe Algorithm in a block-coordinate as an iterative subroutine. However, this slows down overall convergence and suffers from compounding errors when the sub-problems are not fully solved. When stopping early, the primal minimization must be solved to convergence in order to compute the dual function and produce a valid bound. 
%\eric{Mahyar is this correct?}
% In contrast, since our formulation fully separates layers with two sets of variables in \eqref{eq: nn verification problem constrained graph form}, our approach is fully separable 

In contrast to the approach described above, in this paper we used a different variable splitting scheme in \eqref{eq: verification problem split} that allows us to \emph{fully} separate layers in a neural network. This subtle difference has a significant impact: we can efficiently minimize the corresponding augmented Lagrangian in \emph{closed form}, without resorting to any iterative subroutine. Specifically, we use the ADMM algorithm, which is known to converge at an  $O(1/N)$ rate \cite{he20121}. In summary, our method enjoys an order of magnitude faster theoretical convergence, is more robust to numerical errors, and has minimal requirements for parameter tuning. {We remark that during the updates of ADMM, the objective value is not necessarily a lower bound on $J^\star$, and hence, one must run the algorithm until convergence to produce such a bound.} To stop early, we can use a similar strategy as the Frank-Wolfe approach from \cite{bunel2020lagrangian} and run the primal iteration to convergence with fixed dual variables in order to compute the dual function, which is a lower  bound on $J^\star$. %\eric{double check this?}

%
% Using the sequential representation of the neural network in \eqref{eq: DNN model}, we may rewrite the optimization problem in \eqref{eq: maximization problem} as the following constrained optimization problem,
% %
% \begin{alignat}{3} \label{eq: nn verification problem constrained}
% J^\star \leftarrow &\text{minimize} \quad && J(x_{\ell})  \\ \notag
% &\text{subject to } \quad && x_{k+1}=\phi_k(x_{k})  \quad &&k=0,\cdots,\ell-1 \\ \notag
% & \quad && x_0 \in \mathcal{X}.
% \end{alignat}
% %
% with $n:=\sum_{k=0}^{\ell} n_k$ decision variables. This problem is non-convex due to presence of activation layers. \mahyar{To obtain a convex relaxation, we assume that we have 
% access to known lower and upper bounds on $x_k$ of the form $\ell_k \leq x_k \leq u_k$. Denote the graph of $\phi_k$ over $[\ell_k,u_k]$ by $\mathcal{G}_{\phi_k}$,
% \begin{align}
%     \mathcal{G}_{\phi_k} = \{(x_k,x_{k+1}) \mid x_{k+1}= \phi_k(x_k) \ \ell_k \leq x_k \leq u_k\}.
% \end{align}
% }
% We may rewrite \eqref{eq: nn verification problem constrained} equivalently as
% %
% \begin{alignat}{3} \label{eq: nn verification problem constrained graph form}
% J^\star \leftarrow &\text{minimize} \quad && J(x_{\ell})  \\ \notag
% &\text{subject to } \quad && (x_{k},x_{k+1})\in \mathcal{G}_{\phi_k} \quad &&k=0,\cdots,\ell-1 \\ \notag
% & \quad && x_0 \in \mathcal{X}.
% \end{alignat}
% %
% By over-approximating $\mathcal{G}_{\phi_k}$ by a convex set (or ideally by its convex hull), we arrive at a direct layer-wise convex relaxation of the problem. However, this relaxation cannot scale to even medium-sized neural networks. In this section, by exploiting the sequential structure of the constraints, we propose a convex relaxation to \eqref{eq: nn verification problem constrained} that can be split into smaller sub-problems across the layers.

%A direct convex relaxation of \eqref{eq: nn verification problem constrained} cannot scale to even medium-sized neural networks. In this section, by exploiting the sequential nature of the constraints, we propose a convex relaxation to \eqref{eq: nn verification problem constrained} that can be split into smaller sub-problems across the layers.

==> OJCSYS arxiv 0708 submission/conclusion.tex <==
\section{Conclusion}
In this paper, we proposed DeepSplit, a scalable and modular operator splitting technique for solving convex relaxation-based verification problems for neural networks. 
%By splitting the problem into separable sub-problems with analytical or easy-to-compute solutions, 
The method can exactly solve large-scale LP relaxations with GPU acceleration with favorable convergence rates. Our approach leads to tighter bounds across a range of classification and reinforcement learning benchmarks, and can scale to a standard ResNet18. 
%Using this methodology, we can solve LP relaxations exactly and obtain significantly tighter bounds in verification problems for large networks that were previously impossible to solve exactly due to their size. 
%
%Even on relatively small problem instances, our approach can solve LP relaxations almost 7x faster than state-of-the-art commercial solvers with just a single GPU. 
% This speedup can directly accelerate complete verifiers for deep learning by providing tighter and faster solutions to commonly used LP subroutines (e.g. those used in branch-and-bound solvers for MILPs), without needing to rely on excessive computational power. 
%
% Finally, many variations of ADMM have been proposed to improve convergence rates, such as over-relaxation \cite{boyd2011distributed}, adaptive penalty parameter \cite{xu2017adaptive}, and  acceleration techniques \cite{zhang2019accelerating,fu2020anderson}. We leave as future work a further investigation of whether these techniques can also help improve convergence rates in deep learning-sized problem instances, as well as extensions beyond the LP setting. 
%
We leave as future work a further investigation of variations of ADMM that can improve convergence rates in deep learning-sized problem instances, as well as extensions beyond the LP setting. {Furthermore, it would be interesting to extend the proposed method to verification of recurrent neural neworks (RNNs) such as vanilla RNNs, LSTMs\footnote{Long Short-Term Memory.}, and GRUs\footnote{Gated Recurrent Unit.} \cite{ko2019popqorn,ryou2021scalable,mohammadinejad2021diffrnn}.}


%\paragraph{Broader impact \& limitations}
%A limitation of this work is that the tightness of the bounds are not as tight as e.g. SDP solvers or other approaches. This is a necessary trade-off that we make in order to scale to large networks whose LP relaxation was previously impossible to solve, let alone other tighter relaxations. 
%It is possible that users may use our work to argue that their models are robust and thus trustworthy. We emphasize that one should not over-generalize from the robustness guarantees that we enable. Our method, like many others, verify well-defined properties that do not necessarily imply general robustness. 

==> OJCSYS arxiv 0708 submission/defs.tex <==
% Environments
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}    
\newtheorem{remarks}{Remarks}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}    
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}    
\newtheorem{assumption}{Assumption}    
\newtheorem{definition}{Definition}    
\newtheorem{problem}{Problem}    
%\newtheorem*{proof}{Proof}  

% Sets of numbers
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\R}{\mathbb{R}}

% Vectors
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\xbar}{\bar{\x}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bw}{\mathbf{w}}
%\newcommand{\bx}{\mathbf{x}}
%\newcommand{\by}{\mathbf{y}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\tr}{\mathrm{Tr}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bnu}{\boldsymbol{\nu}}
\newcommand{\bxi}{\boldsymbol{\xi}}


\newcommand{\relu}{\mathrm{ReLU}}
\newcommand{\relaxed}{\mathrm{relaxed}}
\newcommand{\proj}{\mathrm{Proj}}

%\newcommand{\vector}{\mathrm{vec}}

% Optimization operators/notation
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\minimize}{minimize \quad}
\DeclareMathOperator*{\maximize}{maximize \quad}
\DeclareMathOperator*{\st}{subject\,\, to \quad}

% Functions
\newcommand{\norm}[1]{\left|\left| #1 \right|\right|}

% Operators
\newcommand{\id}{\text{Id}}
\newcommand{\prox}{\mathbf{prox}}

% For this paper
\newcommand{\Lsq}{L_{\text{sq}}}
\newcommand{\singstate}{
    \begin{bmatrix}
        \x^0 - \xbar^0 \\ \x^1 - \xbar^1
    \end{bmatrix}
}

\def\dom{\mathrm{dom}}


\newcommand{\specialcell}[2][c]{%
	\begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}

\newcommand{\mahyar}[1]{{\color{blue} \noindent #1}}


==> OJCSYS arxiv 0708 submission/experiments.tex <==

\section{Experiments}
\label{sec:experiment}
The strengths of our method are (a) its ability to exactly solve LP relaxations and (b) do so at scales. To evaluate this, we first demonstrate how solving the LP to optimality leads to tighter certified robustness guarantees in image classification and reinforcement learning tasks (Section~\ref{sec:tightness}) compared with the scalable fast linear bounds methods. We then stress test our method in both speed and scalability against a commercial LP solver (Section~\ref{sec:expr_speed}) and in the large network setting, e.g., solving the LP relaxation for a standard ResNet18 (Section~\ref{sec:expr_scalability}). {In Section~\ref{sec:reachability}, we apply our method on reachability analysis of neural network dynamical systems and compare with the state-of-the-art complete verification method $\alpha,\beta$-CROWN~\cite{wang2021beta}.} Section~\ref{sec:expr_residual_balancing} demonstrates the effectiveness of residual balancing in our numerical examples. 

\paragraph{Setup} In all the experiments, we focus on the setting of \emph{verification-agnostic} networks which are networks trained without promoting verification performances, similar to \cite{dathathri2020enabling}. 
% However, we focus on significantly \emph{larger} networks that have previously only been feasibly bounded with fast linear bounds of the LP relaxation \cite{wong2018scaling,xu2020automatic}. 
All the networks have been trained adversarially with the projected gradient descent (PGD) attack~\cite{madry2017towards}. 

In all of the test accuracy certification results reported in this paper, we initialize $\rho = 1.0$ and apply residual balancing when running ADMM. In different experiments, the stopping criterion parameters $\epsilon_\text{abs}, \epsilon_\text{rel}$ of ADMM are chosen by trial-and-error to achieve a balance between the accuracy and the runtime of the algorithm. In all these experiments the objective functions are linear~\cite{kolter2017provable}. Full details about the network architecture and network training can be found in Appendix~\ref{app:expr}. 

\subsection{Improved bounds from exact LP solutions}
\label{sec:tightness}
We first demonstrate how solving the LP exactly with our method results in tighter bounds than prior work that solve convex relaxations in a scalable manner. We consider two main settings: certifying the robustness of classifiers for CIFAR10 and deep Q-networks (DQNs) in Atari games. In both experiments, the pre-activation bounds for formulating the LP verification problem are obtained by the fast linear bounds developed in~\cite{kolter2017provable}.

\paragraph{CIFAR10}
%Much work studying verification in CIFAR10 has focused primarily on a small CNN with only 6k hidden units---smaller than the classic LeNet from MNIST \cite{lecun2015lenet}. In this regime, tighter approaches such as SDP and branch-and-bound are applicable. \shaoru{may need to restrict the discussion to convex relaxation based.}

%Much work studying verification of deep networks in the CIFAR10 setting \cite{singh2019beyond,tjandraatmadja2020convex, de2021scaling}, including the more scalable Lagrangian-based methods \cite{dvijotham2018dual,bunel2020lagrangian}, have focused primarily on a CNN with only 6k hidden units from \cite{kolter2017provable}---smaller than the classic LeNet architecture used for MNIST \cite{lecun2015lenet}. Consequently, the LP relaxation for small networks can be solved exactly with a commercial LP solver such as Gurobi, while alternative approaches such as branch-and-bound \cite{bunel2017unified,bunel2020branch,bunel2020lagrangian} or SDP solvers \cite{dathathri2020enabling} can produce even tighter bounds. 

We consider a convolutional neural network (CNN) of around 60k hidden units whose convex relaxations cannot be feasibly solved by Gurobi (for LP relaxation) or SDP solvers (for the SDP relaxation). Up until this point, the only solutions for large networks were {linear bounds~\cite{wong2018scaling,xu2020automatic} and Lagrangian-based specialized solvers~\cite{dvijotham2018dual, bunel2020lagrangian}} to the LP relaxation.  

%Instead, we consider an order of magnitude larger model, which cannot be feasibly solved by these alternatives.  
%Up until this point, the only solutions for large networks were linear-based bounds to the LP relaxation \cite{wong2018scaling,xu2020automatic}. However, these bounds are known to be quite loose. How much better can we do if we solve the LP exactly? 

%Specifically, we use a large convolutional architecture from~\cite{wong2018scaling}, which is adversarially trained to achieve 43\% robust accuracy against a PGD adversary with $\epsilon=8/255$. Notably, this model is sufficiently large enough to achieve similar performance to the PGD-trained models from \cite{madry2017towards}. Networks of this size have thus far been virtually impossible to certify without using looser bounds of the LP relaxation, and cannot be verified with Gurobi or SDP. 

In Table~\ref{tab:cifar10}, we report the certified accuracy of solving the LP exactly with ADMM in comparison to a range of baselines. Verification of the CNN with $\ell_\infty$ perturbation at the input image with different radii $\epsilon$ is conducted on the $10,000$ test images from CIFAR10, and certified test accuracy is reported as the percentage of verified robust test images by each method. We compare with methods that have previously demonstrated the ability to bound networks of this size: fast bounds of the LP (Linear) \cite{wong2018scaling,xu2020automatic}, and interval bounds (IBP) \cite{gowal2018effectiveness}. We additionally compare to a suite of Lagrangian-based baselines, whose effectiveness at this scale was previously unknown. These methods~\footnote{These Lagrangian-based baselines were implemented using the codes at \url{https://github.com/oval-group/decomposition-plnn-bounds}} include supergradient ascent (Adam)~\cite{bunel2020branch}, dual supergradient ascent (Dual Adam)~\cite{dvijotham2018dual} and a variant thereof (Dual Decomp Adam)~\cite{bunel2020branch}, and a proximal method (Prox)~\cite{bunel2020lagrangian}. As mentioned in Section~\ref{sec:bunel}, these baselines require solving an inner optimization problem through the iterations of the algorithms. In the experiments of Table~\ref{tab:cifar10}, the number of iterations of different algorithms are bounded separately such that each Lagrangian-based method has an average runtime of $9$ seconds to finish verifying one example. Our ADMM solver averages $9$ seconds runtime per example in this verification task, which is the same as the average runtime of the Lagrangian-based methods, with the stopping criterion of $\epsilon_{abs} = 10^{-4}, \epsilon_{rel} = 10^{-3}$ and $\rho$ initialized as $1.0$. 

In Table~\ref{tab:cifar10}, we find that solving the LP exactly leads to consistent gains in certified robustness for large networks, with up to {2\%} additional certified robustness over the best-performing alternative. All the methods in Table~\ref{tab:cifar10} are given the same time budget. Indeed, the better theoretical convergence guarantees of ADMM translate to better results in practice: when given a similar budget, the Lagrangian baselines have worse convergence and cannot verify as many examples.  

\begin{remark}
By Table~\ref{tab:cifar10}, our goal is to compare the performances of ADMM and other Lagrangian-based methods in solving the same LP-based neural network verification problem. The certified test accuracy can be further improved if tighter convex relaxations or the BaB techniques are applied. In fact, for the verification problem considered in Table~\ref{tab:cifar10}, the state-of-the-art neural network verification method $\alpha, \beta$-CROWN~\cite{wang2021beta}, which integrates fast linear bounds methods into BaB, is able to achieve certified test accuracies of $65.4\%, 56.0\%, 37.9\%, 19.9\%$ for $\epsilon = 1/255, 1.5/255, 2/255, 2.5/255$, respectively, given the same $9$s time budget per example. However, as will be shown in Section~\ref{sec:reachability}, our method outperforms $\alpha, \beta$-CROWN in reachability analysis of a neural network dynamical system, which highlights the importance of adapting neural network verification tools for tasks of different structures and scales. 
\end{remark}

\begin{table}[tb]
    \centering
    \caption{Certified test accuracy (\%) of PGD-trained models on CIFAR10 through ADMM, the Lagrangian decomposition methods~\cite{dvijotham2018dual,bunel2020branch}, and fast dual/linear \cite{wong2018scaling,xu2020automatic} or interval bounds \cite{gowal2018effectiveness}. All the LP-based methods (ADMM and Lagrangian) are given the same verification time budget of $9$s per example. The fast linear and IBP bounds can be obtained almost instantly in this experiment, and their achievable certified test accuracy is used for reference.}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lccccccc}
    \toprule
    & Exact & \multicolumn{4}{c}{Lagrangian methods} & \multicolumn{2}{c}{Fast bounds}\\
    \cmidrule(lr){2-2} \cmidrule(lr){3-6} \cmidrule(lr){7-8}
     $\epsilon$ & \hphantom{x} ADMM \hphantom{x} &  \hphantom{x} Adam \hphantom{x} & \hphantom{x} Prox \hphantom{x} & \hphantom{x} Dual Adam \hphantom{x} & \hphantom{x} Dual Decomp Adam \hphantom{x} & \hphantom{x} Linear \hphantom{x} & \hphantom{x} IBP \hphantom{x}\\
     \midrule
     1/255 &  $\mathbf{64.0}$ &  60.5 & 62.4 &   59.8 &  60.3 &  59.8 & 42.8  \\
     1.5/255 & $\mathbf{45.7}$  &  41.2 & 43.5 &   40.5 &   41.1 &  36.8 & 16.8\\
     2/255 & $\mathbf{19.5}$ & 17.3 &  18.2 &  16.9 &  17.1 & 13.2 & 3.6\\
     2.5/255 & $\mathbf{5.5}$  &  4.6 & 4.9 &   4.5 &  4.6 & 3.3 & 0.7 \\
     \bottomrule
\end{tabular} }
    \label{tab:cifar10}
\end{table}

%In addition, the LP dual feasible bound method from~\cite{kolter2017provable} (WK) and IBP (Naive) are applied as well. \todo{Shaoru: Not sure how to introduce these methods in a good way.} With the GPU acceleration, ADMM verifies $30$ examples in a total of $275$ seconds. The average $9.2$ seconds runtime of ADMM is of the same order ($2$ to $10$ seconds) as those of the Lagrangian decomposition methods listed above while ADMM achieves the highest certified test accuracy. The runtime of WK and Naive are mostly less than $0.01$ seconds and in this experiment WK is able to achieve relatively high certified accuracy.



% \paragraph{CIFAR10}
% To highlight the scalability of our approach, we now consider a significantly larger CNN trained on CIFAR10. Specifically, we use a large convolutional architecture from~\cite{wong2018scaling}, which is adversarially trained to achieve 43\% robust accuracy against a PGD adversary with $\epsilon=8/255$. Notably, this model is sufficiently large enough to achieve similar performance to the PGD-trained models from \cite{madry2017towards}. Networks of this size have thus far been virtually impossible to certify without using looser bounds of the LP relaxation, and cannot be verified with Gurobi or SDP. 

% Notably, the network we consider is sufficiently of large capacity to achieve similar performance to the adversarially trained models from \cite{madry2017towards}. Consequently, these networks have thus far been virtually impossible to certify without using looser bounds of the LP relaxation, and cannot be verified with Gurobi or the SDP. 

% We now present the results of LP-ADMM on the CIFAR-10 dataset. 
%ConvNet consisting of four convolutional layers and three fully-connected layers of the connection $4096-512-10$ with ReLU activation after each layer except the last. The channels of the convolutional layers are $(32,64,32,64)$ and strides applied are $(1,2,1,2)$, respectively. 

% In Table \ref{tab:cifar10}, we find that ADMM can significantly improve the number of certified examples. For example, at $\epsilon=2/255$, solving the LP with LP-ADMM can boost certified accuracy by more than 6\% over LP-Dual. % \emph{without} changing the underlying model. 
% These results show, in a large model setting, how the additional tightness in the bound from LP-ADMM can provide substantial gains in certified robustness for adversarially trained models. 


\paragraph{State-robust RL}
We demonstrate our approach on a non-classification benchmark from reinforcement learning: verifying the robustness of deep Q-networks (DQNs) to adversarial state perturbations \cite{zhang2020robust}. Specifically, we verify whether a learned DQN policy outputs stable actions in the discrete space when given perturbed states. Similar to the large network considered in the CIFAR10 setting, this benchmark has only been demonstrably verified with fast but loose linear bounds-based methods\cite{xu2020automatic}. 
%How much tighter can we get with exact LP bounds using ADMM? 
%and are simply too large to be solved with the SDP solver or an LP solver like Gurobi. 

We consider three Atari game benchmarks: BankHeist, Roadrunner, and Pong~\footnote{\cite{zhang2020robust} considers one additional RL setting (Freeway). However, the released PGD-trained DQN is completely unverifiable for nearly all epsilons that we considered.} and verify pretrained DQNs which were trained with PGD-adversarial training~\cite{zhang2020robust}. For each benchmark, we verify the robustness of the DQN over $10,000$ randomly sampled frames as our test dataset. 

Similar to the CIFAR10 setting, we observe consistent improvement in certified robustness of the DQN when solving the LP exactly with ADMM across multiple RL settings. We summarize the results using our method and the linear bounds on LP relaxations~\cite{wong2018scaling,xu2020automatic} in Table \ref{tab:rl}. 


% \begin{table}[t]
%     \vspace{-0.05in}
%     \setlength{\tabcolsep}{5pt}
%     \centering
%     \small
%     \caption{The percentage of actions from a deep Q-network that are certifiably 
%     robust to changes in the state space for various RL tasks.}
%     % \small
%     \begin{tabular}{lcrr>{\bfseries}r}
%     \toprule
%                 &            & \multicolumn{3}{c}{Certifiably robust actions (\%)}\\
%                 \cmidrule{3-5}
%     \textbf{Model} & \textbf{Epsilon} &  \textbf{LP-Dual} &  \textbf{LP-ADMM} &  \textbf{Diff} \\
%     \midrule
%          Bankheist &           0.0016 &               67.0 &               71.4 &            4.3 \\
%                   &           0.0020 &               39.7 &               49.5 &            9.7 \\
%                   &           0.0024 &               12.7 &               25.9 &           13.2 \\
%                   &           0.0027 &                1.4 &                7.3 &            5.9 \\
%     \midrule
%         Roadrunner &           0.0012 &               32.6 &               36.6 &            4.0 \\
%                   &           0.0016 &               26.3 &               27.5 &            1.2 \\
%                   &           0.0020 &               19.6 &               22.8 &            3.1 \\
%                   &           0.0024 &                1.1 &                3.7 &            2.7 \\
%     \midrule
%               Pong &           0.0004 &               96.1 &               97.4 &            1.3 \\
%                   &           0.0008 &               93.4 &               95.6 &            2.2 \\
%                   &           0.0012 &               92.1 &               94.3 &            2.2 \\
%                   &           0.0016 &               82.1 &               84.0 &            1.9 \\
%     \bottomrule
%     \end{tabular}
%     \label{tab:rl}
% \end{table}

% \begin{table}[t]
%     \centering
%     \small
%         \caption{The percentage of actions from a deep Q-network that are certifiably 
%     robust to changes in the state space for various RL tasks.}
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{ccc>{\bfseries}c|ccc>{\bfseries}c|ccc>{\bfseries}c}
%     \toprule
%      \multicolumn{4}{c}{\textbf{Bankheist}} & \multicolumn{4}{c}{\textbf{Roadrunner}} & \multicolumn{4}{c}{\textbf{Pong}} \\
%     \midrule
%     $\epsilon$ & Linear \cite{wong2018scaling,xu2020automatic} & ADMM & Diff & $\epsilon$ & Linear \cite{wong2018scaling,xu2020automatic} & ADMM & Diff & $\epsilon$ & Linear \cite{wong2018scaling,xu2020automatic} & ADMM & Diff  \\
%     \midrule
%     0.0016 &  67.0 & 71.4 & 4.3 & 0.0012 &  32.6 &   36.6 & 4.0 &  0.0004 & 96.1 &  97.4 &  1.3 \\
%      0.0020 &  39.7 &  49.5 &   9.7 &  0.0016 &  26.3 & 27.5 &   1.2 &  0.0008&   93.4 &  95.6 & 2.2 \\
%      0.0024 & 12.7 & 25.9 &   13.2 & 0.0020 &   19.6 &  22.8 & 3.1 & 0.0012 &  92.1 &94.3 & 2.2 \\
%      0.0027 &  1.4 &   7.3 & 5.9 &0.0024 &   1.1 &   3.7 &   2.7 &  0.0016 &82.1 &  84.0 &   1.9 \\
%      \bottomrule
%     \end{tabular} }
%     \label{tab:rl}
% \end{table}


\begin{table*}[t]
    \centering
   \caption{The percentage of actions from a deep Q-network that are certifiably robust to changes in the state space for three RL tasks: Bankheist, Roadrunner, and Pong. We compare fast linear bounds (Linear)~\cite{wong2018scaling,xu2020automatic} and ADMM.}
   \resizebox{\textwidth}{!}{
    \begin{tabular}{ccc|ccc|ccc}
    \toprule
     \multicolumn{3}{c}{Bankheist} & \multicolumn{3}{c}{Roadrunner} & \multicolumn{3}{c}{Pong} \\
    \midrule
    $\epsilon$ & \hphantom{xxxx} Linear \hphantom{xxxx} & ADMM & $\epsilon$ & \hphantom{xxxx} Linear \hphantom{xxxx} & ADMM & $\epsilon$ & \hphantom{xxxx} Linear \hphantom{xxxx} & ADMM  \\
    \midrule
    0.0016 &  67.0 & \textbf{71.4}  & 0.0012 &  32.6 &   \textbf{36.6} &  0.0004 & 96.1 &  \textbf{97.4}  \\
     0.0020 &  39.7 &  \textbf{49.5} &   0.0016 &  26.3 & \textbf{27.5} &   0.0008&   93.4 &  \textbf{95.6}  \\
     0.0024 & 12.7 & \textbf{25.9} &   0.0020 &   19.6 &  \textbf{22.8} & 0.0012 &  92.1 &\textbf{94.3}  \\
     0.0027 &  1.4 & \textbf{7.3} &0.0024 &   1.1 &   \textbf{3.7} &   0.0016 &82.1 &  \textbf{84.0}  \\
     \bottomrule
    \end{tabular} }
    \label{tab:rl}
\end{table*}

% A direct application of our method, DeepSplit, is to exactly solve LP relaxations that verify properties of deep networks (i.e. \cite{ehlers2017formal, kolter2017provable}). We conduct different experiments to evaluate the performance of our splitting method at verifying robustness in image classification and reinforcement learning. Specifically, we certify the robustness of classifiers for MNIST and CIFAR10 and deep Q-networks (DQNs) in Atari games to $\ell_\infty$ perturbations over a range of radii. We compare the certified test accuracy of our approach (LP-ADMM) with the relaxed bound from~\cite{kolter2017provable} (LP-Dual), which computes a dual feasible solution of the LP relaxation. Tables~\ref{tab:vision} and~\ref{tab:rl} present a summary of our results. We focus on the setting of \emph{verification-agnostic} networks, similar to \cite{dathathri2020enabling}. However, our focus is primarily on significantly \emph{larger} networks that could previously only be feasibly bounded with further relaxations of the LP relaxation. All the networks have been trained adversarially with the PGD attack~\cite{madry2017towards}. Full details about the network architecture, network training, and the parameters for our splitting method LP-ADMM can be found in Appendix~\ref{app:expr}. We report the approximate running times for all experiment in Table~\ref{tab:timing}, and show examples of objective convergence for each setting in Figure \ref{fig:admm_obj} with additional plots showing residual convergence in Appendix \ref{app:expr}.  

\subsection{Speed}
\label{sec:expr_speed}
% In this section, we stress test several aspects of DeepSplit for solving LP relaxations. We first measure how it compares to other exact solvers for convex relaxations, namely a commercial LP solver and a specialized SDP solver, in small settings that these solvers can handle. We then push the limits of architecture size and measure the improvement in bounds for a standard ResNet18. 
%
We compare the solving speeds of our method with state-of-the-art solvers for convex relaxations: a commercial-grade LP solver, Gurobi. Since Gurobi cannot handle large networks, we benchmark the approaches on a fully connected network that Gurobi can handle which is an MNIST network with architecture $784 - 600 - 400 - 200 - 100 - 10$ and ReLU activations (see Appendix~\ref{app:expr} for details). 

To demonstrate the effectiveness of GPU-acceleration in the DeepSplit algorithm, we compare the runtime of DeepSplit and Gurobi in solving LP relaxations that bound the output range of the MNIST network with $\ell_\infty$ perturbations in the input. Specifically, for a given example in the MNIST test data set, we apply DeepSplit/Gurobi layer-by-layer to find the tightest pre-activation bounds under the LP-relaxation. 

With the Gurobi solver, we need to solve $2 \times 600$ LPs sequentially to obtain the lower and upper bounds for the first activation layer, $2 \times 400$ LPs for the second activation layer, and so forth. With DeepSplit, the pre-activation bounds can be computed in batch and allows GPU-acceleration. 

In our experiment, we fix the radius of the $\ell_\infty$ perturbation at the input image as $\epsilon = 0.02$. For the Gurobi solver, we randomly choose $10$ samples from the test data set and compute the pre-activation bounds layer-by-layer. The LP relaxation is formulated in CVXPY and solved by Gurobi v9.1 on an Intel Core i7-6700K CPU, which has 4 cores and 8 threads. For each example, the total solver time of Gurobi is recorded with the average solver time being $275.9$ seconds. For the DeepSplit method, we compute the pre-activation bounds layer-by-layer on $19$ randomly chosen examples. The algorithm applies residual balancing with the initial $\rho = 1.0$ and the stopping criterion is given by $\epsilon_\text{abs} = 10^{-4}, \epsilon_\text{rel}= 10^{-3}$. The total running time of DeepSplit is $717.9$ seconds, with $37.8$ seconds per example on average. With the GPU-acceleration, our method achieves 7x speedup in verifying NN properties compared with the commercial-grade Gurobi solver. 



% We additionally find that our LP solver is 30x faster than the SDP solver \cite{dathathri2020enabling}. Specifically, we can solve LP relaxations at 0.2 hours per thousand examples, whereas the SDP relaxation takes 6 hours per thousand examples. 
% This highlights the trade-off in speed and scalability of solving different relaxations: SDPs can produce tighter bounds but LPs are substantially faster to solve.


% We first compare the solving speeds of our method with state-of-the-art solvers for convex relaxations of deep networks: a commercial-grade LP solver, Gurobi, and specialized SDP-solvers \cite{dathathri2020enabling}. We benchmark these exact solvers on two tasks: calculating intermediate bounds on a fully connected network that Gurobi can handle, and verifying a small convolutional architecture that the SDP-solver can handle (see Appendix~\ref{app:speed} for further details on experimental setup). 
% We compare the solving speeds on networks that are small enough such that the corresponding convex relaxations can be solved exactly by other means. Specifically, for the MNIST data set, we consider the following settings: (i) a fully-connected network with architecture $784-600-400-200-100-10$ (MNIST-A), whose LP relaxation can be solved with the Gurobi solver, and (ii) a small convolutional architecture (MNIST-B) whose SDP relaxation can be solved using a specialized GPU-based SDP solver \cite{dathathri2020enabling}. The results are as follows.

% We compare our method with that of Gurobi, a highly optimized commercial-grade solver for LPs. Specifically, we compute lower and upper bounds for the pre-activations in the network for the fully connected network. This is a common procedure in complete verification approaches, such as branch-and-bound algorithms for MILP \cite{bunel2020branch}. 
%We first find that our method provides a nearly 7x speedup over commercial-grade LP solvers. On average, it takes ADMM 38 seconds per example to calculate these intermediate bounds using a single GeForce GTX 1080, in comparison to 258 seconds per example for Gurobi on an Intel Core i7-6700K. %We note that the potential speedup is even larger since due to the small size of the network, the ADMM was not fully utilizing the GPU. %Even on these small problem instances, we find that our approach provides a nearly 7x speedup over commercial LP solvers. Further discussion of these timing experiments can be found in Appendix \ref{app:timing}. 
%We additionally find that our LP solver is 30x faster than the SDP solver \cite{dathathri2020enabling}. Specifically, we can solve LP relaxations at 0.2 hours per thousand examples, whereas the SDP relaxation takes 6 hours per thousand examples. 
% For example, it took our method (LP-ADMM) approximately 20 hours to verify all 10,000 MNIST test set images at 10 different epsilon values. In contrast, the SDP relaxation \cite{raghunathan2018semidefinite} takes 3 hours to verify 500 examples at one epsilon value---30x slower than solving the LP. 
%This highlights the trade-off in speed and scalability of solving different relaxations: SDPs can produce tighter bounds but LPs are substantially faster to solve.

% We find that our method is significantly faster than solving the convex relaxation through other approaches. For example, it took our method (LP-ADMM) approximately 20 hours to verify all MNIST test set images for the convolutional architecture at 10 different epsilon values (\ref{tab:timing}), taking on average 2 hours per epsilon to verify all 10,000 examples. See \ref{app:timing} for the running time summary of each experiment. In contrast, the SDP relaxation \cite{raghunathan2018semidefinite} takes 3 hours to verify 500 examples at one epsilon value for a similarly sized CNN. This highlights the difference in speed and scalability of solving the LP relaxation over the SDP one, albeit at the cost of looser verification guarantees. 

% $\bullet$ We also compared the runtime of ADMM with that of Gurobi, a highly optimized commercial-grade solver for LPs. Specifically, we compute lower and upper bounds for the pre-activations in the network for the fully connected network. This is a common procedure in complete verification approaches, such as branch-and-bound algorithms for MILP \cite{bunel2020branch}. We find that, on average, it takes ADMM 38 seconds per example to calculate these intermediate bounds using a single GeForce GTX 1080, in comparison to 258 seconds per example for Gurobi on an Intel Core i7-6700K. Even on these small problem instances, we find that our approach provides a nearly 7x speedup over commercial LP solvers. Further discussion of these timing experiments can be found in Appendix \ref{app:timing}. 

% \begin{figure}
% \begin{subfigure}{0.45 \columnwidth}
%     \includegraphics[width = \linewidth]{admm_lirpa_lb_compare.eps}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.45 \columnwidth}
%     \includegraphics[width = \linewidth]{admm_lirpa_ub_compare.eps}
% \end{subfigure}
%     \caption{ResNet18 output lower (left) and upper (right) bounds obtained using either ADMM (blue dots) and LiRPA (orange triangles). Higher lower bounds and lower upper bounds are better. For ease of visualization, bounds are sorted in ascending order according to the ADMM bound.}
%     \label{fig:admm_lirpa}
% \end{figure}

\begin{figure}
	\centering
\begin{subfigure}{0.45 \columnwidth}
    \includegraphics[width = \linewidth]{new_lb_hist.pdf}
\end{subfigure}
\hfill
\begin{subfigure}{0.45 \columnwidth}
    \includegraphics[width = \linewidth]{new_ub_hist.pdf}
\end{subfigure}
    \caption{A total of $1000$ ResNet18 output lower and upper bounds are computed from ADMM and LiRPA for comparison in CIFAR10. Histograms of the relative improvement percentage of ADMM over LiRPA are shown for the lower (top) and upper (bottom) bounds, which have an average relative improvement of $31.61\%$ and $2.32\%$, respectively.}
    \label{fig:admm_lirpa}
\end{figure}

\subsection{Scalability}
\label{sec:expr_scalability}
To test the scalability and generality of our approach, we consider solving the LP relaxation for a ResNet18, which up to this point has simply not been possible due to its size. The only applicable method here is LiRPA~\cite{xu2020automatic}---a highly scalable implementation of the linear bounds that works for arbitrary networks but can be quite loose in practice. For this experiment, we measure the improvement in the bound from solving the LP exactly in comparison to LiRPA.

The ResNet18 network is trained on CIFAR10 whose max pooling layer is replaced by a down-sampling convolutional layer for comparison with LiRPA~\cite{xu2020automatic}~\footnote{The max pooling layer has not been considered in the implementation of LiRPA by the submission of this paper. Codes of LiRPA are available at \url{https://github.com/KaidiXu/auto_LiRPA} under the BSD 3-Clause "New" or "Revised" license.} which is capable of computing provable linear bounds for the outputs of general neural networks and is the only method available so far that can handle ResNet18. The ResNet18 is adversarially trained using the fast adversarial training code from \cite{wong2020fast}. 

In our experiments, for the first $100$ test examples in CIFAR10, we use LiRPA to compute the preactivation bounds for each ReLU layer in ResNet18 and then apply ADMM to compute the lower and upper bounds of ResNet18 outputs (there are $10$ outputs corresponding to the $10$ classes of the dataset). The ADMM is run with stopping criterion $\epsilon_{abs} = 10^{-5}, \epsilon_{rel} = 10^{-4}$. With $\ell_\infty$ ball input perturbation of radius $\epsilon  = 1/255$, we find that exact LP solutions with our ADMM solver can produce substantial improvements in the bound at ResNet18 scales, as shown in Figure~\ref{fig:admm_lirpa}. For a substantial number of examples, we find that ADMM can find significantly tighter bounds (especially for lower bounds). 

{
\subsection{Reachability analysis of dynamical systems}
\label{sec:reachability}
We consider over-approximating the reachable sets of a discrete-time neural network dynamical system $x(t+1) = f_{NN}(x(t))$ over a finite horizon where $x(t) \in \mathbb{R}^{n_x}$ denotes the state at time $t=0,1,\cdots$, $f_{NN}$ is a feed-forward neural network, and $n_x$ is the dimension of the system. Specifically, we consider a cart-pole system with $4$ states under nonlinear model predictive control~\cite{lucia2017rapid}, and train a $4-100-100-4$ neural network $f_{NN}(x)$ with ReLU activations to approximate the closed-loop dynamics with sampling time $0.05 s$. The $4$ states $x = [x_1 \ x_2 \ x_3 \ x_4]^\top$ of the cart-pole system represent the position and velocity of the cart, and the angle and angular speed of the pendulum, respectively. Given an initial set $\mathcal{X}_0 \subset \mathbb{R}^4$ such that $x(0) \in \mathcal{X}_0$, we want to over-approximate the reachable set of $x(t) = f_{NN}^{(t)}(x(0))$ where $f_{NN}^{(t)}$ denotes the $t$-th order composition of $f_{NN}$ and is a feed-forward neural network itself.  

Over-approximating $x(t)$ can be formulated as a neural network verification problem~\eqref{eq: maximization problem} where $f = f_{NN}^{(t)}$ is given by the sequential concatenation of $t$ copies of $f_{NN}$ and the input set $\mathcal{X}$ is chosen as the initial set $\mathcal{X}_0$. A box approximation of $x(t)$ can be obtained by minimizing/maximizing the $i$-th output of the neural network $f^{(t)}_{NN}$ for $1 \leq i \leq n_x = 4$.

With a randomly chosen initial set $x(0) \in \mathcal{X}_0 = \{x \mid x_1 \in [-1.8 \ -1.6] \ \textrm{m}, x_2 \in [0.5 \ 0.7] \ \textrm{m/s}, x_3 \in [0.035 \ 0.105]\ \textrm{rad}, x_4 \in [0.2 \ 0.4]\ \textrm{rad/s}\}$, we consider the horizon $t = 20$ and compute a box over-approximation of the reachable set of $x(20)$ through both DeepSplit and the state-of-the-art BaB-based verification method $\alpha, \beta$-CROWN~\cite{wang2021beta} \footnote{Codes of $\alpha,\beta$-CROWN are available at \url{https://github.com/huanzhang12/alpha-beta-CROWN} under the BSD 3-Clause "New" or "Revised" license.}. From $1000$ simulated trajectories with uniformly sampled initial states from $\mathcal{X}_0$, the emperically estimated lower and upper bounds for $x(20)$ are given by $[-1.74 \ 0.14 \ -0.10 \ 0.022]^\top \leq x(20) \leq [-0.91 \ 0.92 \ -0.036 \ 0.11]^\top$. With the time budget $1470$s per bound, the box over-approximations of $x(20)$ given by DeepSplit and $\alpha,\beta$-CROWN are given as follows:
\begin{equation*}
\begin{aligned}
     \textrm{DeepSplit:} &
    \begin{bmatrix}
    -4.19 \\ -4.39 \\ -2.14 \\ -3.88
    \end{bmatrix} \leq x(20) \leq 
    \begin{bmatrix}
    3.00 \\ 4.81 \\ 1.99 \\ 3.91
    \end{bmatrix}, \\
    \alpha, \beta \textrm{-CROWN}: &
    % \begin{bmatrix}
    % -514.77 \\ -626.83 \\ -319.09 \\ -656.38
    % \end{bmatrix} \leq x(20) \leq 
    % \begin{bmatrix}
    % 499.98 \\ 672.83 \\ 311.44 \\ 650.26
    % \end{bmatrix}. 
        \begin{bmatrix}
    -38.38 \\ -46.52 \\ -23.85 \\ -55.97
    \end{bmatrix} \leq x(20) \leq 
    \begin{bmatrix}
    37.08 \\ 48.58 \\ 22.86 \\ 48.21
    \end{bmatrix}.
\end{aligned}
\end{equation*}
We observe that DeepSplit gives a reasonable over-approximation of the reachable set of $x(20)$, while the bounds obtained by $\alpha,\beta$-CROWN in this task are an order of magnitude more conservative. Such comparison result holds for other randomly chosen initial sets $\mathcal{X}_0$ too. The details of the experimental setup is shown in Appendix~\ref{app:expr}.

% \begin{remark}
% Through the reachability analysis example, we want to highlight that different methods for solving the verification problem have their own preferable operation regimes in terms of verification goal, neural network architecture, size, etc. Indeed, $\alpha,\beta$-CROWN achieves outstanding performances in verifying the robustness of the image classifiers. In Table~\ref{tab:cifar10}, we only compare LP-based verification methods and linear bounds propagation methods whose tightness is limited by their formulations, e.g., the use of fixed pre-activation bounds and the inherent conservatism due to the convex relaxation. Given the same $9$s time budget, $\alpha, \beta$-CROWN achieves certified test accuracies of $65.4\%, 56.0\%, 37.9\%, 19.9\%$ for $\epsilon = 1/255, 1.5/255, 2/255, 2.5/255$, respectively, which significantly outperform all the methods mentioned in Table~\ref{tab:cifar10}. In this work, we aim to propose a candidate method for solving the LP-based neural network verification problem at scale. Integrating our proposed method into BaB or tighter convex relaxation formulations~\cite{ singh2019beyond, tjandraatmadja2020convex} (see discussion in Appendix~\ref{sec:tighter_relaxation}) is left for future work.  
% \end{remark}
}


\subsection{Effects of residual balancing}
\label{sec:expr_residual_balancing}
We demonstrate the effects of residual balancing on the convergence of ADMM through the MNIST network (see Appendix~\ref{app:expr} for details). We conduct our experiment on the $1938$-th example which is randomly chosen from the MNIST test dataset. For this example, the MNIST network predicts its class (number $4$) correctly. We add an $\ell_\infty$ perturbation of radius $\epsilon = 0.02$ to the input image and verify if the network outputs are robust with respect to class number $3$. {This corresponds to setting $i^\star = 4,i = 3$ and $\mathcal{X} = \{x \mid \lVert x - x^* \rVert_\infty \leq 0.02 \}$ in problem~\eqref{eq:class_verify} where $x^*$ denotes the chosen test image.}

The maximum number of iterations is restricted to $3000$. The objective values, primal and dual residuals of ADMM for the network under different fixed augmentation parameters $\rho$ are plotted in Figure~\ref{fig:mnist_fc4}. The residual balancing in this experiment is applied with $\tau = 2$, $\mu = 10$, and $\rho$ initialized as $10.0$. 

\begin{figure*}[tb]
	\centering
	\begin{subfigure}{0.32\textwidth}
		\centering
		\includegraphics[width=\linewidth]{mnist_fc4_obj.pdf}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.32\textwidth}
		\centering
		\includegraphics[width=\linewidth]{mnist_fc4_p_res.pdf}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.32 \textwidth}
		\centering
		\includegraphics[width = \linewidth]{mnist_fc4_d_res.pdf}
	\end{subfigure}
	\caption{The objective values (left), primal residuals (middle), and dual residuals (right) of ADMM under different augmentation parameters $\rho$ on the fully connected MNIST  network described in Appendix~\ref{app:expr}. }
	\label{fig:mnist_fc4}
\end{figure*}

The effects of $\rho$ on the convergence rates of the primal and dual residuals are illustrated empirically in Figure~\ref{fig:mnist_fc4}. Despite initialized at a large value $10.0$, residual balancing is able to adapt the value of $\rho$ and achieves significant improvement in convergence rate compared with the case of constant $\rho = 10.0$. As observed in our other experiments, with residual balancing, ADMM becomes insensitive to the initialization of $\rho$ and usually achieves a good convergence rate. 

% Although ADMM has convergence guarantees for its objective values, primal and dual residuals, it may take too many iterations for ADMM to achieve a solution of high accuracy~\cite{boyd2011distributed}.


%the lower/upper bounds of ADMM from these $100$ examples are arranged in an ascending order in Figure~\ref{fig:admm_lirpa_full} and are compared with those obtained by LiRPA. We observe that the bounds from ADMM are consistently tighter than those from LiRPA. The average running time of ADMM across the $100$ examples is $2312$ seconds. Overall bound statistics are shown in Table \ref{tab:scalability}. 



==> OJCSYS arxiv 0708 submission/intro.tex <==
\section{Introduction}
%
%Lack of formal guarantees on the performance of neural networks is a serious limitation that precludes their adoption in safety-critical domains. Recent studies show that neural networks are vulnerable to adversarial attacks \cite{szegedy2013intriguing}. This drawback has spurred a lot interest in developing tools that can verify various properties of neural networks or build defense mechanisms against adversarial attacks. 
%
%Due to their ability to capture complex dependencies, neural networks have been  tremendously useful in a variety of vision and reinforcement learning tasks. However, neural network lack formal guarantees on their performance, which preclude their use in safety-critical domains. Indeed, recent studies show that neural networks are vulnerable to adversarial attacks \cite{szegedy2013intriguing} or more generally, input perturbations. %For example, in deep reinforcement learning tasks, small perturbations to sensor inputs (from natural noise or adversarial examples) are often enough to change network-based decisions. 
%In light of these drawbacks, there has been an increasing interest in developing tools that can verify various properties of neural networks or build defense mechanisms against adversarial attacks. 
%
%For example, in the context of image classification using deep networks, it is desirable to verify that all points in the vicinity of a correctly-classified example would be classified correctly (local robustness). Similarly, in deep reinforcement learning tasks, it would be useful to choose a robust action under a worst-case deviation in input space due to possible adversaries or noise in the observed states \cite{everett2020certified}.

Despite their superior performance, neural networks lack formal guarantees, raising serious concerns about their adoption in  safety-critical applications such as autonomous vehicles \cite{cao2019adversarial} and medical machine learning \cite{finlayson2019adversarial}. Motivated by this drawback, 
%
%Motivated by the vulnerability of neural networks to adversarial attacks, 
there has been an increasing interest in developing tools to verify desirable properties for neural networks, such as robustness to adversarial attacks.

%For example, in the context of image classification using deep networks, it is desirable to verify that all points in the vicinity of a correctly-classified example would be classified correctly (local robustness). Similarly, in deep reinforcement learning tasks, it is desirable to choose a robust action under a worst-case deviation in input space due to possible adversaries or noise in the observed states \cite{lutjens2020certified}.
%

Neural network verification refers to the problem of verifying whether the output of a neural network satisfies certain properties for a bounded set of input perturbations. This problem can be framed as optimization problems of the form
%
\begin{align} \label{eq: maximization problem}
J^\star \leftarrow \mathrm{minimize} \quad J(f(x)) \quad \text{subject to}  \quad x \in \mathcal{X},
\end{align}
%
where $f$ is given by a deep neural network, $J$ is a real-valued function representing a performance measure (or a specification), and $\mathcal{X}$ is a set of inputs to be verified. In this formulation, verifying the neural network amounts to certifying whether the optimal   value of \eqref{eq: maximization problem} is bounded below by a certain threshold. 

{As an example, consider a classification problem with $n_f$ classes, in which for a data point $x \in \mathbb{R}^{n_x}$, $f(x) \in \mathbb{R}^{n_f}$ denotes the vector of scores for all the classes. The classification rule is $C(x) = \argmax_{1 \leq i \leq n_f} e_i^\top f(x)$ where $e_i$ denotes the $i$-th standard basis. Given a correctly classified $x^\star \in \mathbb{R}^{n_x}$ and a perturbation set $\mathcal{X} \subset \mathbb{R}^{n_x}$ that contains $x$, we say that $f$ is locally robust at $x^\star$ with respect to $\mathcal{X}$ if $C(x)=C(x^\star)$ for all $x \in \mathcal{X}$. Verifying the local robustness at $x^\star$ then amounts to verifying that the optimal values of the following $n_f-1$ optimization problems
% % %
\begin{align} \label{eq:class_verify}
    \underset{x \in \mathcal{X}}{\operatorname{minimize}} &\quad (e_{i^\star} - e_i)^\top f(x), \quad i \neq i^\star,
\end{align}
are positive, where $i^\star=C(x^\star)$ is the class index of $x^\star$. Problem \eqref{eq:class_verify} is an instance of \eqref{eq: maximization problem} where $J$ is a linear function.} 
%

Problem \eqref{eq: maximization problem} is large-scale and non-convex, making it extremely difficult to solve efficiently--both in terms of time and memory. 
%
%Indeed, for neural networks with $\relu$\footnote{Rectified Linear Unit.} activation functions and linear performance measures, \eqref{eq: maximization problem} can be formulated as a Mixed-Integer Linear Program (MILP), which is combinatorial in nature. To mitigate the inefficiency of global solvers, several past works have proposed convex relaxations to \eqref{eq: maximization problem} for various activation functions, where the goal is to find \emph{guaranteed lower bounds} on the objective function. Depending on the activation function and nature of the over-approximation, one can obtain a hierarchy of convex relaxations with varying degree of tightness.
%Notable works are Linear Programming (LP) relaxation of \cite{kolter2017provable} and SDP relaxations of \cite{raghunathan2018certified,raghunathan2018semidefinite,fazlyab2019probabilistic}. 
%However, even for reasonably-sized neural networks, these relaxations are not tractable, and must be replaced by even weaker relaxations in practice, which lead to vacuous bounds.
%
For $\relu$ activation functions and linear objectives, the problem in \eqref{eq: maximization problem} can be cast as a Mixed-Integer Linear Program (MILP) \cite{lomuscio2017approach,cheng2017maximum,dutta2018output,fischetti2018deep}, which can be solved for the global solution via, for example, Branch-and-Bound (BaB) methods. While  we  do  not  expect  these  approaches  to  scale  to  large problems,  for  small  neural  networks they can still be practical.
%These methods generally work by recursively splitting the feasible set into multiple parts and solving the problem restricted in each subdivision, typically via relaxation techniques such as Linear Programming (LP). 
%Although the practical convergence can be greatly improved by using a tighter relaxations, this formulation is computationally intractable for large neural networks and/or for large input sets.
%\eric{I don't think we need to say this much about MILPs in our introduction. We can probably shorten this to "this can be solved as an MILP with branch and bound, but this is intractable for large networks"}

Instead of solving \eqref{eq: maximization problem} for its global minimum, one can instead find \emph{guaranteed lower bounds} on the optimal value via convex relaxations, such as Linear Programming (LP) \cite{kolter2017provable} and Semidefinite Programming (SDP) \cite{raghunathan2018semidefinite,fazlyab2019efficient,fazlyab2020safety}. 
%
Verification methods based on convex relaxations are sound but incomplete, i.e., they are guaranteed to detect all {false negatives} but also produce false positives, whose rate depends on the tightness of the relaxation. 
%
Although convex relaxations are polynomial-time solvable (in terms of number of decision variables), in practice they are not computationally tractable for large-scale neural networks. To improve scalability, these relaxations must typically be further relaxed \cite{kolter2017provable,weng2018towards,zhang2018efficient,dvijotham2018dual,bunel2020lagrangian}.

\paragraph{Contributions} 
%
In this work, we propose an algorithm to solve LP relaxations of \eqref{eq: maximization problem} for their global solution and for large-scale feed-forward neural networks.
%
%In this work, we propose an algorithm for solving convex relaxations \emph{exactly} for large-scale neural networks. 
%
%
Our starting point is to express \eqref{eq: maximization problem} as a constrained optimization problem whose constraints are imposed by the forward passes in the network. We then introduce additional decision variables and consensus constraints that naturally split the corresponding problem into independent subproblems, which often have closed-form solutions. %These additional variables and constraints can be interpreted as introducing fictitious ``identity layers'' in between the actual layers of the network. 
Finally, we employ an operator splitting technique based on the Alternating Direction Method of Multipliers (ADMM)~\cite{boyd2011distributed}, to solve the corresponding Lagrangian relaxation of the problem. 
%
This approach has several favorable properties. First, the method requires minimal parameter tuning and relies on simple operations, which scale to very large problems and can achieve a good trade-off between runtime and solution accuracy. Second, all the solver operations are amenable to fast parallelization with GPU acceleration. Third, our method is fully modular and applies to standard network architectures. 

We employ our method to compute exact solutions to LP relaxations on the worst-case performance of adversarially trained deep networks, with a focus on networks whose convex relaxations {are difficult} to solve due to their size. Specifically, we perform extensive experiments in the $\ell_\infty$ perturbation setting, where we verify robustness properties of image classifiers for CIFAR10 and deep Q-networks (DQNs) in Atari games \cite{zhang2020robust}. Our method is able to solve LP relaxations at scales that are too large for exact {MILP} verifiers, SDP relaxations, or commercial LP solvers such as Gurobi. {We also demonstrate the use of our method in  computing reachable set over-approximations of a neural network dynamical system over a long horizon, where our method is compared with the state-of-the-art BaB method~\cite{wang2021beta}.}

\subsection{Related work}
%There is an extensive literature on verifying properties of deep networks. Here, we focus primarily on describing most closely related work studying convex relaxations and complete verifiers that use these convex relaxations as a subroutine. Other approaches for verifying deep networks include bound propagation, dual verifiers \cite{dvijotham2018dual}, randomized smoothing \cite{cohen2019certified, croce2019provable, yang2020randomized}, and abstract interpretations \cite{gehr2018ai2, singh2018fast, singh2019beyond}. 

\paragraph{Convex relaxations} 
LP relaxations are relatively the most scalable form of convex relaxations \cite{ehlers2017formal}. However, even solving LPs can become computationally prohibitive for small convolutional networks \cite{salman2019convex}.
%
%Most closely related are methods which provide certified bounds on the output of deep network using a form of convex relaxation.
%
One line of work studies computationally cheaper but looser bounds of the LP relaxation \cite{kolter2017provable}, which {we denote as linear bounds}, and have been extended to larger and more general networks and settings \cite{wong2018scaling, weng2018towards, zhang2018efficient, xu2020automatic}. These bounds tend to be loose unless optimized during training, which typically comes at a significant cost to standard performance. Further work has aimed to tighten these bounds \cite{singh2019beyond,tjandraatmadja2020convex, de2021scaling}, however these works focus primarily on small convolutional networks and struggle to scale to more typical deep networks. Other work has studied the limits of these convex relaxations on these small networks using vast amounts of CPU-compute \cite{salman2019convex}. Recent SDP-based approaches \cite{dathathri2020enabling} can produce much tighter bounds on these small networks. 

\paragraph{Lagrangian-based bounds}
Related to our work is that which solves the Lagrangian of the LP relaxation \cite{dvijotham2018dual,bunel2020lagrangian}, which can tighten the bound but do not aim to solve the LP exactly due to relatively slow convergence.
However, these works primarily study small networks whose LP relaxation can still be solved exactly with Gurobi. Although these works could in theory be used on larger networks, only the faster, linear bounds-based methods \cite{xu2020automatic} have demonstrated applicability to standard deep learning architectures. In our work, we solve the LP relaxation exactly in \emph{large} network settings that previously have only been studied with loose bounds of the LP relaxation such as LiRPA \cite{xu2020automatic}. 
% For these networks, it is not possible to solve the LP relaxation exactly with off-the-shelf LP solvers and the SDP solver cannot scale. 
%However, these methods have been primarily studied in the context of small networks whose LP relaxations can still be solved exactly with Gurobi. 
% Of these works, only \cite{xu2020automatic} has been applied to large networks; the rest have been primarily studied on small networks whose LP relaxation can still be solved exactly with Gurobi. 
%Only \cite{xu2020automatic} has applied their approach to large networks typically used in deep learning. In contrast, in our work, we focus on the \emph{large} network setting 
%Another line of work has expanded the SDP relaxation to more general architectures \cite{raghunathan2018semidefinite, fazlyab2020safety}, problems beyond safety verification \cite{} and more scalable solvers \cite{dathathri2020enabling}. 

% Compared to LP relaxations, SDPs provide tighter bounds.
% However, to obtain accurate solutions, these SDP relaxations must be solved via interior-point method solvers that rely on matrix factorization, and thus cannot scale to large networks or problems with large input dimensions. Furthermore, the tightness of these relaxations is highly influenced by the pre-activation bounds used to narrow down the relaxation domain. In \cite{dathathri2020enabling}, the authors propose a sub-gradient based method to solve an SDP relaxation of the problem that relies on forward and backward pass operations on the network. Although more scalable, sub-gradient methods are far slower than second-order methods.
%
%Compared to LP relaxations, SDPs can achieve tighter bounds but are still computationally expensive for small convolutional networks. 
% In relation to these works, our approach allows us to directly and efficiently solve the LP relaxation at significantly larger scales to get tighter bounds on networks that are still too large for existing SDP solvers. 


\paragraph{Operator splitting methods} 
Operator splitting, and in particular the ADMM method, is a powerful technique in solving structured convex optimization problems and has applications in numerous settings ranging from optimal control \cite{o2013splitting} to training neural networks \cite{taylor2016training}. These methods scale well with the problem dimensions, can exploit sparsity in the problem data efficiently \cite{zheng2017fast}, are amenable to parallelization on GPU \cite{schubiger2020gpu}, and have well-understood convergence properties under minimal regularity assumptions \cite{boyd2011distributed}. The benefit of ADMM as an alternative to interior-point solvers has been shown in various classes of optimization problems \cite{o2016conic}. Our operator splitting method is specifically tailored for neural network verification in order to fully exploit the problem structure.


\paragraph{Complete verification methods} 
These methods verify properties of deep networks exactly (i.e., they find the optimal value $J^\star$ and a global solution $x^\star$) using methods such as Satisfiability Modulo Theories (SMT) solvers \cite{scheibler2015towards,ehlers2017formal,katz2017reluplex} and MILP solvers \cite{lomuscio2017approach, cheng2017maximum, dutta2018output, fischetti2018deep}. Complete verification methods typically rely on BaB algorithms \cite{bunel2017unified}, in which the verification problem is divided into subproblems (branching) that can be verified using incomplete verification methods (bounding) \cite{bunel2020branch}. However, these methods have a worst-case exponential runtime and have difficulty scaling beyond relatively small convolutional networks. Motivated by this, several recent works have been reported on improving the scalability of BaB methods by developing custom solvers in the bounding part to compute cheaper intermediate bounds and hence, speed up their practical running time \cite{bunel2020lagrangian,de2021improved, xu2021fast, wang2021beta}. {In the same spirit, our proposed method for solving the large-scale LP relaxations can be potentially used as a bounding subroutine in BaB for complete verification which we leave for future research. }


%Motivated by this, several recent works have improved the practical running time of BaB methods with custom solvers for medium-sized networks \cite{bunel2020lagrangian,de2021improved, xu2021fast, wang2021beta}, \shaoru{but have yet to scale to larger deep networks.}


\paragraph{Notation} We denote the set of real numbers by $\mathbb{R}$, the set of nonnegative real numbers by $\mathbb{R}_{+}$, the set of real $n$-dimensional vectors by $\mathbb{R}^n$, the set of $m\times n$-dimensional real-valued matrices by $\mathbb{R}^{m\times n}$, 
%the $m$-dimensional vector of all ones by $\mathrm{1}_m$, 
%the $m\times n$-dimensional zero matrix by $0_{m\times n}$, 
and the $n$-dimensional identity matrix by $I_n$. 
%We denote by $\mathbb{S}^{n}$, $\mathbb{S}_{+}^n$, and $\mathbb{S}_{++}^n$ the sets of $n$-by-$n$ symmetric, positive semidefinite, and positive definite matrices, respectively. 
The $p$-norm ($p \geq 1$) is denoted by $\|\cdot\|_p \colon \mathbb{R}^n \to \mathbb{R}_{+}$. 
%For $A \in \mathbb{R}^{m\times n}$, the inequality $A \geq 0$ is element-wise. 
%
%For $A \in \mathbb{S}^n$, the inequality $A \succeq 0$ means $A$ is positive semidefinite. 
%
For a set $\mathcal{S}$, we define the indicator function $\mathbb{I}_{\mathcal{S}}(x)$ of $\mathcal{S}$ as $\mathbb{I}_{\mathcal{S}}(x)=0$ if $x \in \mathcal{S}$ and $\mathbb{I}_{\mathcal{S}}(x)= +\infty$ otherwise. Given a function  $f \colon \mathcal{X} \to \mathcal{Y}$, the graph of $f$ is the set $\mathcal{G}_{f} = \{(x,f(x)) \mid x \in \mathcal{X}\}$.



